A Survey of Pre-trained Language Models for Processing Scientific Text

The number of Language Models (LMs) dedicated to processing scientific text is on the rise. Keeping pace with the rapid growth of scientific LMs (SciLMs) has become a daunting task for researchers. To date, no comprehensive surveys on SciLMs have been undertaken, leaving this issue unaddressed. Given the constant stream of new SciLMs, appraising the state-of-the-art and how they compare to each other remain largely unknown. This work fills that gap and provides a comprehensive review of SciLMs, including an extensive analysis of their effectiveness across different domains, tasks and datasets, and a discussion on the challenges that lie ahead.

==> tables/backup_main_tables.tex <==


\begin{table}

  \caption{
  Existing LMs for scientific text. 
  \textbf{Arch.} denotes Architecture information.
  In the \textbf{Objective} column, 
  \textit{MLM} denotes Masked Language Model,  
  \textit{NSP} denotes Next Sentence Prediction, and   \textit{SOP} denotes Sentence Order Prediction.
  % 
  In the \textbf{Type} column, \textit{CP} and \textit{FS} denote Continual Pretraining and From Scratch, respectively. 
  %
 In the \textbf{Domain} column,  \textbf{CS} represents computer science, \textbf{Bio} represents Biomedical domain, \textbf{Chem} represents Chemical domain, and \textbf{Multi} represents multiple domains. 
It is noted that the date information is chosen from the first date the paper appears on the Internet.
%  
  }
  \label{table_lms_1} 
      \resizebox{\textwidth}{!}{%
  % \setlength\tabcolsep{-5pt}
  \begin{tabular}{l l l l c c c c c c }



% 
    \toprule
  \textbf{No.} &  \textbf{Date} & \textbf{Model} & \makecell[l]{\textbf{Type of} \\ \textbf{Arch.} }  & \textbf{Architecture} &  \textbf{Training Objective} & \makecell{\textbf{Type of} \\ \textbf{Pre-training} } & \makecell{\textbf{Model} \\ \textbf{Size}} & \textbf{Domain} &  \textbf{Pre-training Corpus}  \\



  
    \midrule
 1 &   2019/01 & BioBERT \cite{10.1093/bioinformatics/btz682} & En & BERT & MLM, NSP & CP & 110M & Bio & PubMed \\ \midrule
 
    
2  &   2019/02 & BERT-MIMIC \cite{10.1093/jamia/ocz096} & En & BERT & MLM, NSP & CP & \makecell{110M \& 340M} & Bio & MIMIC-III  \\ \midrule

    
3  &   2019/03 & SciBERT \cite{beltagy-etal-2019-scibert}  & En & BERT & MLM, NSP & CP \& FS & 110M & CS + Bio & Semantic Scholar Corpus \\ \midrule

    
4  &   2019/04 & BioELMo \cite{jin-etal-2019-probing} & Others & ELMo & Bi-LM & FS & 93.6M & Bio & PubMed  \\ \midrule


5   &   2019/04 & Clinical BERT (Emily)  \cite{alsentzer-etal-2019-publicly} & En & BERT & MLM, NSP & CP & 110M & Bio & MIMIC-III \\ \midrule


6    &   2019/04 & ClinicalBERT (Kexin) \cite{Huang2019ClinicalBERTMC} & En  & BERT & MLM, NSP & CP & 110M & Bio & MIMIC-III  \\ \midrule

    
7  &   2019/06 & BlueBERT \cite{peng-etal-2019-transfer} & En & BERT & MLM, NSP & CP & \makecell{110M \& 340M} & Bio & PubMed + MIMIC-III \\  \midrule


8 &    2019/06 & G-BERT \cite{ijcai2019p0825} & Others & \makecell{GNN \\ + BERT} & \makecell{Self-Prediction, \\ Dual-Prediction} & CP & 3M & Bio & MIMIC-III \\ \midrule


9 &    2019/07 & BEHRT \cite{7801} & En & BERT & MLM, NSP & CP & N/A & Bio & \makecell{Clinical Practice Research Datalink}  \\ 
\midrule

    
10 &    2019/08 & BioFLAIR \cite{sharma2019bioflair} & Others & Flair & Bi-LM & CP & N/A & Bio & PubMed \\ \midrule
    
11 &   2019/09 & EhrBERT \cite{info:doi/10.2196/14830} & En & BERT & MLM, NSP & CP & 110M & Bio & Electronic Health Record Notes \\  \midrule


12 &   2019/11 & S2ORC-SciBERT \cite{lo-etal-2020-s2orc} & En & BERT & MLM, NSP & FS & 110M & Multi  & S2ORC \\ \midrule

    
13 &   2019/12 & Clinical XLNet \cite{huang-etal-2020-clinical} & Others & XLNet & \makecell{Generalized Autoregressive \\ Pretraining}  & CP & 110M & Bio & MIMIC-III \\ \midrule


14 &   2020/02 & SciGPT2 \cite{luu-etal-2021-explaining} & De & GPT2 & LM & CP & 124M & CS &  S2ORC \\ \midrule


15 &   2020/03 & NukeBERT \cite{jain2020nukebert} & En &  BERT & MLM, NSP  & CP & 110M & Chem & NText \\ \midrule



16 &   2020/04 & GreenBioBERT \cite{poerner-etal-2020-inexpensive} & En & BERT & \makecell{CBOW Word2Vec, \\ Word Vector Space Alignment} & CP & 110M & Bio & PubMed + PMC \\  \midrule


17 &   2020/04 & SPECTER \cite{cohan-etal-2020-specter} & En & BERT & Triple-Loss & CP & 110M  & Multi &  Semantic Scholar Corpus \\ \midrule


18 & 2020/05  & BERT-XML \cite{zhang2020bertxml} & En & BERT  & MLM, NSP &  FS  & N/A & Bio & Electronic Health Record Notes \\ \midrule


19 &  2020/05 &	Bio-ELECTRA \cite{ozyurt-2020-effectiveness} & En & ELECTRA & Replaced Token Prediction & FS & 14M & Bio & PubMed + PMC \\  \midrule

 
20 &   2020/05 & Med-BERT \cite{Rasmy2020MedBERTPC} & En & BERT & \makecell{MLM, \\ Prolonged LOS Prediction}  & FS & 110M & Bio & Cerner Health Facts (Version 2017)  \\ \midrule
    


21 &   2020/05 & ouBioBERT \cite{2005.07202} & En & BERT & MLM, NSP & FS & 110M & Bio & PubMed \\ \midrule



22 & 2020/07  & PubMedBERT \cite{10.1145/3458754} & En & BERT & \makecell{MLM,  NSP, \\ Whole-Word Masking} & FS   & 110M & Bio & PubMed \\ \midrule



23 & 2020/08  & MC-BERT \cite{zhang2020conceptualized} & En &  BERT & MLM, NSP &  CP  & \makecell{110M \& 340M} & Bio & \makecell{Chinese Biomedical Community QA \\ + Chinese Medical Encyclopedia \\ + Chinese Electric Medical Record} \\ \midrule



24 & 2020/09  & BioALBERT \cite{article_naseem} & En & ALBERT & MLM, SOP   &  CP  & \makecell{12M \& 18M} & Bio & PubMed + PMC \\ \midrule


25 & 2020/09  & BRLTM \cite{9369833} & En & BERT  & MLM &    FS  & N/A & Bio & Private Electronic Health Record \\ \midrule


26 &  2020/10 & BioMegatron \cite{shin-etal-2020-biomegatron} & En &  Megatron & MLM, NSP &  CP \& FS  & \makecell{345M \& \\  800M \& 1.2B} & Bio & PubMed + PMC \\ \midrule


27  &    2020/10  &    CharacterBERT \cite{el-boukkouri-etal-2020-characterbert} & En &  BERT + Character-CNN & MLM, NSP & FS & 105M & Bio & MIMIC-III  + PubMed \\ \midrule


28 & 2020/10  & ChemBERTa \cite{chithrananda2020chemberta} & En & RoBERTa & MLM &  FS  & 125M & Chem & SMILES from PubCHEM \\ \midrule



29 &  2020/10 & ClinicalTransformer \cite{10.1093/jamia/ocaa189} & En & \makecell{BERT \\ ALBERT \\ RoBERTa \\ ELECTRA} & \makecell{MLM, NSP \\ 
MLM, SOP \\
MLM \\
Replaced Token Prediction} & CP   & \makecell{110M \\ 
12M \\
125M \\
110M} & Bio &  MIMIC-III \\ \midrule

30 & 2020/10  & SapBERT \cite{liu-etal-2021-self} & En & BERT & Multi-Similarity Loss &  CP  & 110M &  Bio &   UMLS  \\  \midrule




31 & 2020/10  & UmlsBERT \cite{michalopoulos-etal-2021-umlsbert} & En & BERT  &  MLM &  CP  & 110M &  Bio & MIMIC-III  \\ \midrule



32  &    2020/11  &   bert-for-radiology \cite{10.1093/bioinformatics/btaa668}  & En &    BERT & MLM, NSP & CP \& FS &  110M & Bio & Chest Radiograph Reports \\  \midrule


33 &    2020/11 & Bio-LM \cite{lewis-etal-2020-pretrained}  & En & RoBERTa & MLM & FS & \makecell{125M \& 355M} & Bio & PubMed + PMC + MIMIC-III \\ \midrule



 34 &    2020/11  &    CODER \cite{yuan2021coder} & En &   \makecell{PubMedBERT \\ 
mBERT} & Contrastive Learning & CP & \makecell{110M \\ 110M} & Bio & UMLS \\ \midrule

 


35  &    2020/11  &    exBERT \cite{tai-etal-2020-exbert}  & En & BERT & MLM, NSP  & CP & N/A & Bio & ClinicalKey + PMC  \\ \midrule


36  &    2020/12  &    BioMedBERT \cite{chakraborty-etal-2020-biomedbert}  & En &    BERT & MLM, NSP & CP \& FS & 340M & Bio & BREATHE Dataset v1.0 \\  \midrule



37  &    2020/12  &    LBERT \cite{article_warikoo} & En &  BERT & MLM, NSP & CP & 110M & Bio & PubMed  \\   \midrule





38  &    2021/03  &    OAG-BERT \cite{10.1145/3534678.3539210}  & En & BERT & MLM & FS & 110M & Multi & AMiner + PubMed    \\ \midrule




39  &    2021/04  &    CovidBERT \cite{Hebbar_Xie_2021} & En &    BERT & MLM, NSP & CP & 110M & Bio & Covid-19 Related Corpora \\ \midrule




40  &    2021/04  &    ELECTRAMed \cite{miolo2021electramed} & En  &    ELECTRA  & Replaced Token Prediction & FS & N/A & Bio & PubMed \\ \midrule

  


41  &    2021/04  &    KeBioLM  \cite{yuan-etal-2021-improving}  & En &    PubMedBERT & \makecell{MLM, Entity Detection, \\ Entity Linking} & CP & 110M & Bio & \makecell{Pubmed Docs \\ from PubMedDS} \\  \midrule


  
42  &    2021/04  &    SINA-BERT \cite{taghizadeh2021sinabert} & En  &  BERT & MLM & CP & 110M & Bio & \makecell{Manually Collected \\ (2.8M Documents)}   \\  


  \bottomrule
\end{tabular}
}

\end{table}


\begin{table}

  \caption{
  A continuation of the table from Table~\ref{table_lms_1}. 
%   Existing LMs for scientific text. 
%   \textbf{Arch.} denotes Architecture information.
%   In the \textbf{Objective} column, 
%   \textit{MLM} denotes Masked Language Model,  
%   \textit{NSP} denotes Next Sentence Prediction, and   \textit{SOP} denotes Sentence Order Prediction.
%   % 
%   In the \textbf{Type} column, \textit{CP} and \textit{FS} denote Continual Pretraining and From Scratch, respectively. 
%   %
%  In the \textbf{Domain} column,  \textbf{CS} represents computer science, \textbf{Bio} represents Biomedical domain, \textbf{Chem} represents Chemical domain, and \textbf{Multi} represents multiple domains. 
% It is noted that the date information is chosen from the first date the paper appears on the Internet.
%  
  }
  \label{table_lms_2} 

      \resizebox{\textwidth}{!}{%
  \begin{tabular}{l l l l c c c c c c }



  
  %   \toprule
  % \textbf{No.} &  \textbf{Date} & \textbf{Model} & \textbf{Arch.} & \textbf{Base-model} & \textbf{Objective} & \textbf{Type} & \textbf{Size} & \textbf{Domain} & \textbf{Corpora}  \\ 


    \toprule
  \textbf{No.} &  \textbf{Date} & \textbf{Model} & \makecell[l]{\textbf{Type of} \\ \textbf{Arch.} }  & \textbf{Architecture} &  \textbf{Training Objective} & \makecell{\textbf{Type of} \\ \textbf{Pre-training} } & \makecell{\textbf{Model} \\ \textbf{Size}} & \textbf{Domain} &  \textbf{Pre-training Corpus}  \\


  



\midrule
43  &    2021/05  &  MathBERT (Peng) \cite{peng2021mathbert}  & En  &   BERT  & \makecell{MLM, Masked Substructure Prediction, \\ Context Correspondence Prediction} & CP & 110M & Math & \makecell{Formula-Context Pairs \\ Extracted from arXiv} \\ \midrule


44  &    2021/05  &   NukeLM \cite{burke2021nukelm} & En  & \makecell{BERT \\ RoBERTa-Base \\ RoBERTa-Large} & MLM & CP & \makecell{110M \\ 125M \\  355M} & Chem & \makecell{U. S. Department of \\ Energy Office Scientific and \\ 
Technical Information Database} \\ \midrule 


45  &    2021/05  &    ProteinBERT \cite{10.1093/bioinformatics/btac020} & Others &  BERT &  Corrupted Token, Annotation Prediction & FS & 16M & Bio & UniProtKB/UniRef90 + GO \\ \midrule


46 &    2021/05  &    SciFive  \cite{phan2021scifive} & En-De  & T5 & Span Corruption Prediction  & CP & \makecell{220M  \\ \&  770M} & Bio & PubMed + PMC \\ \midrule


47  &    2021/06  &    BioELECTRA \cite{kanakarajan-etal-2021-bioelectra} & En &   ELECTRA & Replaced Token Prediction & CP \& FS & 110M & Bio & PubMed + PMC \\ \midrule


48  &    2021/06  &    ChemBERT \cite{doi:10.1021/acs.jcim.1c00284}  & En &  RoBERTa & MLM & CP & 110M  & Chem & 
ACS Publications \\ \midrule 


49  &    2021/06  &    EntityBERT \cite{lin-etal-2021-entitybert} & En & BERT  & Entity-Centric MLM & CP & 110M   & Bio & MIMIC \\ \midrule 



50  &    2021/06  & MathBERT (Shen) \cite{shen2023mathbert} & En & RoBERTa & MLM &  CP & 110M & Math & \makecell{Mathematics Curricula \\  + Mathematics Textbooks \\ + Mathematics Course Syllabi \\ + Mathematics Paper Abstracts} \\ \midrule


  
51  &    2021/07  &    MedGPT  \cite{kraljevic2021medgpt} & De &  \makecell{GPT2 + GLU \\ + RotaryEmbed}  & LM & CP & N/A & Bio &  Electronic Health Record Notes \\ \midrule 


52  &    2021/08  &    SMedBERT  \cite{zhang2021smedbert} & Others & SMedBERT & \makecell{Masked Neighbor Modeling, SOP, \\
Masked Mention Modeling, MLM} & FS & N/A & Bio & DXY BBS (Bulletin Board System)  \\ \midrule 




53  &    2021/09  &  Bio-cli \cite{carrino2021biomedical} & En & RoBERTa & \makecell{MLM, Subword Masking \\ or Whole Word Masking} & FS & 125M & Bio & Clinical Corpus + Biomedical Corpus \\ \midrule 





54  &    2021/09  &    MatSciBERT \cite{gupta2022matscibert} & En &  BERT & MLM & CP & 110M & Chem & Material Science Corpus \\ \midrule 


55  &    2021/10  &    ClimateBert  \cite{webersinke2022climatebert} & En & DistilROBERTA & MLM & CP & 66M & Climate & \makecell{News Articles  + Research Abstracts \\ + Corporate Climate Reports} \\ \midrule 





  
56  &    2021/10  &    MatBERT \cite{Trewartha2022-sl} & En &  BERT & MLM & FS & 110M & Chem &  \makecell{Peer-Reviewed Materials \\ Science Journal Articles} \\ \midrule 



 



57  &    2021/11  &   UTH-BERT \cite{aclinical_kawazoe}  & En  & BERT & MLM, NSP & FS & 110M & Bio & \makecell{Clinical Texts from The \\ University of Tokyo Hospital}   \\ \midrule 



58  &    2021/12  &    ChestXRayBERT \cite{9638337} & En  &  BERT & MLM, NSP & CP & 110M & Bio & 20617 Scientific Papers in PMC  \\ \midrule 
% Chest Radiology





59  &    2021/12  &    MedRoBERTa.nl \cite{Verkijk_Vossen_2021}  & En &   RoBERTa & MLM & FS & 123M & Bio & \makecell{Dutch Hospital Notes, from EHRs} \\ \midrule 



60  &    2021/12  &    PubMedELECTRA \cite{TINN2023100729}  & En &   ELECTRA & Replaced Token Prediction & FS & \makecell{110M \\ \& 335M} & Bio & PubMed  \\ \midrule 



% 61  &    2022/01  &    \makecell[l]{Clinical-BigBird \\ Clinical-Longformer} \cite{li2022clinicallongformer}  & En &  \makecell{BigBird \\ Longformer}  & MLM & CP & \makecell{166M \\ 149M}  & Bio & MIMIC-III  \\ \midrule 
61  &    2022/01  &   Clinical-Longformer  \cite{li2022clinicallongformer}  & En &  \makecell{BigBird \\ Longformer}  & MLM & CP & \makecell{166M \\ 149M}  & Bio & MIMIC-III  \\ \midrule 
  
  
62 &    2022/03 & BioLinkBERT \cite{yasunaga-etal-2022-linkbert} & En  & BERT & \makecell{MLM, \\ Document Relation Prediction}  & FS & \makecell{110M \\ \& 340M} & Bio  & PubMed + PMC \\  \midrule 
 



63  &    2022/04  &    BioBART  \cite{yuan-etal-2022-biobart}  & En-De &  BART  & \makecell{Text Infilling,\\ Sentence Permutation} & CP & \makecell{140M \\ \& 400M} & Bio & PubMed  \\ \midrule 



  
64  &    2022/04  &    SecureBERT  \cite{1a3e2a1ca6f94c7589c870bc0b3e1e31}  & En & RoBERTa & MLM & CP & 125M & Cybersecurity & \makecell{Manually Collected \\ (98,411 Documents)}   \\ \midrule 



65   &    2022/05  &    BatteryBERT \cite{doi:10.1021/acs.jcim.2c00035}  & En &  BERT & MLM & CP \& FS & 110M & Chem & \makecell{Battery-Related Scientific Papers \\ from RSC, Elsevier, Springer} \\ \midrule 




66  &    2022/05  &   bsc-bio-ehr-es  \cite{carrino-etal-2022-pretrained}  & En &  RoBERTa & MLM & FS & 125M & Bio & \makecell{Electronic Health Record Corpus
\\ + Biomedical Corpus} \\ \midrule 


67   &    2022/05  &    ChemGPT  \cite{frey2022neural}  & De & GPT & Autoregressive LM & FS & 1B & Chem & SMILES from PubCHEM \\ \midrule 


68  &    2022/05  &    PathologyBERT \cite{santos2022pathologybert}   & En &  BERT & MLM, NSP & FS & 110M & Bio &  \makecell{Manually Labeled Pathology Reports \\
+ Unlabeled Pathology Reports from EUH} \\ \midrule 





69  &    2022/05  &    ScholarBERT \cite{hong2023diminishing}   & En & BERT &  MLM & FS & 770M & Multi & Public Resource Dataset \\ \midrule 



  
70 &    2022/06 & RadBERT \cite{yan2022radbert}  & En & RoBERTa & MLM & CP & 110M & Bio &  Radiology Reports \\ \midrule



71  &    2022/06  &    SciDeBERTa \cite{jeong2022scideberta}  & Others &  DeBERTa &  MLM & CP & N/A & Multi & S2ORC \\  \midrule 
  

72  &    2022/06  &    SsciBERT \cite{10.1007/s11192-022-04602-4} & En & BERT & MLM, NSP & CP & 110M & Social Science  & Collected from Web of Science \\  \midrule



73 &    2022/06 & ViHealthBERT \cite{minh-etal-2022-vihealthbert} & En & PhoBERT & \makecell{MLM, NSP, \\ Capitalized Prediction} & CP & 110M & Bio & \makecell{OSCAR Dataset \\ + Their Text Mining Corpus} \\  \midrule 




74  &    2022/07  &    Clinical Flair \cite{rojas-etal-2022-clinical}  & Others &  \makecell{Flair} & Character-Level Bi-LM & CP & N/A & Bio & Free-Text Diagnostic Suspicions \\  \midrule 


75  &    2022/08  &    KM-BERT  \cite{Kim2022-er}  & En &  BERT & MLM, NSP & CP & 99M & Bio &  \makecell{Medical Textbooks \\ + Health Information News \\ + Medical Research Articles}  \\ \midrule





76  &    2022/08  &    MaterialsBERT (Shetty) \cite{Shetty_2023}  & En  &  PubMedBERT & MLM, NSP, Whole-Word Masking & CP & 110M & Chem &  Polymer Scholar  \\ \midrule 


77   &    2022/08  &    ProcessBERT \cite{KATO2022957}  & En &  
 BERT & MLM, NSP & CP & 110M & Chem & ChemECorpus  \\ \midrule 



78 &    2022/09 & BioGPT \cite{10.1093/bib/bbac409}  & De & GPT & Autogressive LM & FS & \makecell{347M  \\ \& 1.5B} & Bio & PubMed \\ \midrule



79  &    2022/09  &    ChemBERTa-2 \cite{ahmad2022chemberta}  & En &  RoBERTa &  MLM, Multi-Task Regression & FS & 125M & Chem & SMILES from PubCHEM   \\   \midrule


80  &    2022/09  & CSL-T5   \cite{li-etal-2022-csl}  & En-De &   T5 & \makecell{Fill-in-the-blank-style \\ Denoising Objective} & FS & 220M & Multi & Chinese Academic Journals \\  \midrule 



81  &    2022/09  &    MaterialBERT (Yoshitake) \cite{yoshitake2022materialbert} & En  &  BERT & MLM, NSP & FS & 110M &  Chem & Scientific Articles from NIMS \\  \midrule




82  &    2022/10  & AcademicRoBERTa \cite{yamauchi-etal-2022-japanese} & En & RoBERTa & MLM & FS & 125M & Multi & CiNii Articles \\  \midrule



 83  &    2022/10  & Bioberturk \cite{PPR:PPR560833} & En & BERT & MLM, NSP & CP \& FS & N/A & Bio & \makecell{Turkish Medical Articles \\ +
Turkish Radiology Thesis} \\ 




  






  \bottomrule
\end{tabular}
}

\end{table}


\begin{table}
  \caption{
  A continuation of the table from Table~\ref{table_lms_1} and Table~\ref{table_lms_2}. 
  %
%   Existing LMs for scientific text. 
%   \textbf{Arch.} denotes Architecture information.
%   In the \textbf{Objective} column, 
%   \textit{MLM} denotes Masked Language Model,  
%   \textit{NSP} denotes Next Sentence Prediction, and   \textit{SOP} denotes Sentence Order Prediction.
%   % 
%   In the \textbf{Type} column, \textit{CP} and \textit{FS} denote Continual Pretraining and From Scratch, respectively. 
%   %
%  In the \textbf{Domain} column,  \textbf{CS} represents computer science, \textbf{Bio} represents Biomedical domain, \textbf{Chem} represents Chemical domain, and \textbf{Multi} represents multiple domains. 
% It is noted that the date information is chosen from the first date the paper appears on the Internet.
%  
  }
  \label{table_lms_3} 
  \setlength{\tabcolsep}{1.5pt}
      \resizebox{\textwidth}{!}{%
  \begin{tabular}{l l l c c c c c c c }

  
  %   \toprule
  % \textbf{No.} &  \textbf{Date} & \textbf{Model} & \textbf{Arch.} & \textbf{Base-model} & \textbf{Objective} & \textbf{Type} & \textbf{Size} & \textbf{Domain} & \textbf{Corpora}  \\ 


    \toprule
  \textbf{No.} &  \textbf{Date} & \textbf{Model} & \makecell[l]{\textbf{Type of} \\ \textbf{Arch.} }  & \textbf{Architecture} &  \textbf{Training Objective} & \makecell{\textbf{Type of} \\ \textbf{Pre-training} } & \makecell{\textbf{Model} \\ \textbf{Size}} & \textbf{Domain} &  \textbf{Pre-training Corpus}  \\




\midrule
84  &    2022/10  &    DRAGON \cite{yasunaga2022deep}  & Others &  GreaseLM & \makecell{MLM, KG Link Prediction} & CP & 360M & Bio & PubMed + UMLS KG \\  \midrule



85  &    2022/10  &    UCSF-BERT \cite{sushil2022developing} & En  &   BERT & MLM, NSP & FS & 135M & Bio &  Clinical Notes of UCSF Health  \\ \midrule 


86  &    2022/10  & ViPubmedT5 \cite{phan2023enriching} & En-De & T5 & Spans-masking Learning & CP & 220M & Bio & ViPubmed \\ \midrule




87 &    2022/11 & Galactica \cite{taylor2022galactica} & De & GPT & Autogressive LM & FS & \makecell{125M \\ \& 1.3B \& 6.7B \\ \& 30B \& 120B} & Multi &  \makecell{Papers, Reference Material, Knowledge Bases, \\Common Crawl, Code, <work> Datasets} \\ 
\midrule



  
88  &    2022/11  &    VarMAE \cite{hu-etal-2022-varmae} & En &  RoBERTa & MLM & CP & 110M & Multi  & \makecell{Semantic Scholar Corpus \\ + Finance-Related Online Platforms}  \\ \midrule



89  &    2022/12  &    AliBERT \cite{berhe-etal-2023-alibert} & En & BERT & MLM & FS & 110M & Bio & \makecell{Drug Database 550MB + Cochrane 27MB  + \\
 Articles 4300MB  + Thesis 300MB 
+ RCP 2200MB}  \\ \midrule


90 &    2022/12 & BioMedLM \cite{cite_BioMedLM}  & De & GPT2 & Autogressive LM & FS & 2.7B &  Bio  &  PubMed + PMC \\ \midrule


  
91  &    2022/12  &    BioReader \cite{frisoni-etal-2022-bioreader} &  Others & T5 + RETRO & MLM & CP & 229.5M & Bio & PubMed  \\ \midrule




92  &    2022/12  &    ClinicalT5 \cite{lu-etal-2022-clinicalt5} &  En-De & T5 & Span-mask Denoising Objective  & CP & \makecell{220M \\ \& 770M} & Bio & MIMIC-III  \\ \midrule


93  &    2022/12   & CySecBERT \cite{bayer2022cysecbert} & En & BERT & MLM, NSP & CP & 110M  & Cybersecurity & \makecell{Blog Data + arXiv Data + Twitter Data \\ + National Vulnerability Database} \\ \midrule



94  &    2022/12  &    GatorTron \cite{Yang2022-pf} & En & BERT & MLM & FS & 8.9B & Bio &  \makecell{De-identified Clinical Notes \\ + PubMed + Wikipedia}  \\ \midrule



95  &    2022/12   & Med-PaLM \cite{singhal2023large} & De & Flan-PaLM & Instruction Prompt Tuning & CP & 540B & Bio & N/A \\ \midrule

  
% from here

96  &    2023/01  &    Clinical-T5 \cite{Clinical_T5_lehman} & En-De &  T5   & \makecell{Fill-in-the-blank-style \\ Denoising Objective} & \makecell{CP \& FS} & \makecell{220M \\ \& 770M}  & Bio & MIMIC-III + MIMIC-IV  \\ \midrule


% 97  &    2023/01  &    \makecell[l]{CPT-BigBird \\ CPT-Longformer} \cite{Louisa_heyarticle}  & En &  \makecell{BigBird \\ Longformer}  & MLM & CP & \makecell{166M \\ 149M}  & Bio & Senior Scholars' Basket of Journals  \\ \midrule 
97  &    2023/01  &    CPT-BigBird \cite{Louisa_heyarticle}  & En &  \makecell{BigBird \\ Longformer}  & MLM & CP & \makecell{166M \\ 149M}  & Bio & Senior Scholars' Basket of Journals  \\ \midrule 

98  &    2023/01  &   ProtST  \cite{xu2023protst}  & En &  BERT   & \makecell{Masked Protein Modeling \\ + Contrastive Learning \\
+ Multi-modal Masked Prediction} & CP \& FS  &  N/A  &  Protein  &  ProtDescribe  \\ \midrule


99  &    2023/01  &  SciEdBERT   \cite{liu2023context}  & En  &  BERT   & MLM & CP  & 110M &  Science Education &  \makecell{The Academic Journal Dataset \\ + Students’ Responses}   \\ \midrule




100  &    2023/02  &    Bioformer \cite{fang2023bioformer}  & En &  BERT   & MLM, NSP & FS & 43M & Bio & PubMed + PMC   \\ \midrule


101  &    2023/02  &   Lightweight Clinical Transformers  \cite{rohanian2023lightweight}  & En  &  DistilBERT   &  \makecell{MLM, \\ Knowledge Distillation Objective} & CP  & \makecell{15M \& 18M \\ \& 25M \& 65M} & Clinical & MIMIC-III   \\ \midrule




102  &    2023/03  &    ManuBERT \cite{ManuBERT_kumar} & En & BERT & MLM & CP & \makecell{110M  \\ \& 126M} & Manufaturing & \makecell{Manufacturing Process Journals \\ + Six Commonly Used Textbooks}  \\ \midrule 



103  &    2023/03  &   RAMM  \cite{yuan2023ramm}  & En &  PubmedBERT   & \makecell{MLM, Image-Text Matching, \\ Image-Text Contrastive Learning} & CP  & N/A & Bio & ROCO, MIMIC-CXR, PMCPM   \\ \midrule



104  &    2023/04  &  DrBERT  \cite{labrak2023drbert} &  En &  RoBERTa & MLM & FS & 110M & Bio & \makecell{Online Sources \\ + Private Hospital Stays Reports}  \\ \midrule 


105  &    2023/04  &  MOTOR   \cite{lin2023medical}  & Others  &  BLIP   & \makecell{MLM, Image-Text Matching, \\ Image-Text Contrastive Learning} &  CP   &  N/A & Bio &   MIMIC-CXR \\ \midrule




106  &    2023/05  &   BiomedGPT \cite{zhang2023biomedgpt} & En-De &  BART & \makecell{Text Infilling,\\ Sentence Permutation} & FS & \makecell{33M \\ \& 93M \\ \& 182M}  & Bio &  \makecell{CheXpert + PathVQA + Retinal Fundus \\ + International Skin Imaging Collaboration \\  + Peir Gross   + CytoImageNet + MIMIC-III \\ + DeepLesion + NCBI BioNLP Corpus \\ + MedICaT + PubMed + SLAKE + IU X-ray  } \\ \midrule 


107  &    2023/05  &   Patton  \cite{jin-etal-2023-patton}  & Others  &  GNN-nested Transformer  & \makecell{Network-contextualized MLM,  \\ Masked Node Prediction} & CP  & N/A &  Multi &  \makecell{Academic Networks from Microsoft Academic Graph, \\ E-commerce Networks from Amazon}  \\ \midrule


108  &    2023/05  &  TurkRadBERT \cite{türkmen2023harnessing} & En & BERT & MLM, NSP & CP \& FS & 110M & Bio &  \makecell{General Turkish Corpus + Head CT Reports \\ + Turkish Biomedical Corpus \\ 
+ Turkish Electronic Radiology Theses} \\ \midrule


109  &    2023/06  &   CamemBERT-bio  \cite{touchent2023camembertbio}  & En & CamemBERT    & Whole Word Masking  & CP  &  111M & Bio &  Biomed-fr: ISTEX, CLEAR, and E3C  \\ \midrule



110  &    2023/06  &   ClinicalGPT \cite{wang2023clinicalgpt} & De & T5 & \makecell{Supervised Fine Tuning \\ 
Rank-based Training} & \newupdate{Instruction Tuning} & \newupdate{CP} & Bio & Supervised Task Datasets  \\  \midrule


% 111  &    2023/06  &   \makecell[l]{EriBERTa \\ EriBERTa-Longformer}  \cite{delaiglesia2023eriberta}  &  En &  \makecell{RoBERTa \\ Longformer}   & MLM & CP \& FS  & \makecell{125M \\ 149M} & Bio &  \makecell{MIMIC-III, EMEA, ClinicalTrials, PubMed, \\ SNOMED-CT, SPACCC,  UFAL, Wikipedia Med, \\ Private Clinical Documents, Medical Crawler}  \\ \midrule
111  &    2023/06  &   EriBERTa  \cite{delaiglesia2023eriberta}  &  En &  \makecell{RoBERTa \\ Longformer}   & MLM & CP \& FS  & \makecell{125M \\ 149M} & Bio &  \makecell{MIMIC-III, EMEA, ClinicalTrials, PubMed, \\ SNOMED-CT, SPACCC,  UFAL, Wikipedia Med, \\ Private Clinical Documents, Medical Crawler}  \\ \midrule


112  &    2023/06  &  K2   \cite{deng2023k2}  & De &  LLaMA   & Cosine Loss   & CP  & 7B & Geoscience &  \makecell{Geoscience-Related Wikipedia Pages, \\ 
Open-access Geoscience Papers, \\
Geoscience Paper’s Abstracts}   \\ \midrule



113  &    2023/06  &    PharmBERT \cite{10.1093/bib/bbad226}  & En &  BERT   & MLM & CP  & 110M & Bio &  DailyMed  \\ \midrule

%%%%

114  &    2023/07  &    BioNART \cite{asada-miwa-2023-bionart}  & En-De &  BERT   & Connectionist Temporal Classification & CP  & 110M &  Bio &  PubMed/MEDLINE   \\ \midrule


115  &    2023/07  &    BIOptimus \cite{pavlova-makhlouf-2023-bioptimus}  & En &  BERT   & MLM & CP  & 110M & Bio &  PubMed   \\ \midrule




116  &    2023/07  &    KEBLM \cite{LAI2023104392}  & En &  BERT & \makecell{MLM, Ranking Objective, \\
Contrastive Learning}  & CP  & N/A  & Bio &   UMLS, PubChem, MSI  \\ \midrule




117  &    2023/08  &    GIT-Mol \cite{liu2023gitmol}  & Others &  \makecell{\newupdate{BLIP2}}   & \makecell{Xmodal-Text Matching, \\ 
Xmodal-Text Contrastive Learning}  &  N/A &  700M & Chem &  PubChem \\ 




% 118  &    2023/08  &    icsBERTs \cite{LIU2023127}  & En & BERT &  \makecell{Business Word Masking, \\ Multi-Task Learning, \\ Sentence Structural Objective}   & CP & 110M  & Business &   \rewrite{Manually Collected}   \\



  \bottomrule
\end{tabular}
    }

\end{table}



==> tables/dataset_kbs.tex <==
\begin{table}[ht]
\centering
\caption{Knowledge Bases in Scientific Domains}
\begin{tabular}{|c|c|}
\hline
\textbf{Scientific Domain} & \textbf{Knowledge Base} \\
\hline
Biology & Gene Ontology (GO) \\
& KEGG (Kyoto Encyclopedia of Genes and Genomes) \\
& UniProtKB (Universal Protein Resource) \\
\hline
Chemistry & ChEBI (Chemical Entities of Biological Interest) \\
& PubChem \\
& ChemSpider \\
\hline
Physics & INSPIRE-HEP (High-Energy Physics Literature Database) \\
& NIST Physics Laboratory Database \\
& Astrophysics Data System (ADS) \\
\hline
Medicine & SNOMED CT (Systematized Nomenclature of Medicine) \\
& MeSH (Medical Subject Headings) \\
& DrugBank \\
\hline
Earth Sciences & GeoNames \\
& USGS EarthExplorer \\
& WorldClim (Global Climate Data) \\
\hline
Mathematics & MathSciNet \\
& Zentralblatt MATH \\
& EuDML (European Digital Mathematics Library) \\
\hline
Environmental Science & ENVO (Environment Ontology) \\
& EDGG (European Dry Grassland Group) Database \\
& EPA Envirofacts Data Warehouse \\
\hline
\end{tabular}
\end{table}


==> tables/dataset_kbs_general.tex <==
\begin{table}[ht]
\centering
\caption{Popular Knowledge Bases in the General Domain}
\begin{tabular}{|c|c|}
\hline
\textbf{Knowledge Base} & \textbf{Description} \\
\hline
Wikidata & Collaboratively edited KB linked to Wikipedia \\
\hline
DBpedia & Extracts structured data from Wikipedia \\
\hline
Freebase & Open, collaborative KB acquired by Google \\
\hline
YAGO & Multilingual KB with information from multiple sources \\
\hline
WordNet & Lexical database for English words and relationships \\
\hline
NELL & Never-Ending Language Learner for web-mined knowledge \\
\hline
ConceptNet & Multi-lingual KB representing common-sense knowledge \\
\hline
BabelNet & Multilingual KB integrating WordNet and Wikipedia \\
\hline
OpenCyc & Large KB with structured common-sense knowledge \\
\hline
\end{tabular}
\end{table}

==> tables/dataset_ner_re.tex <==



\begin{table}

  \caption{Existing NER and RE datasets in scientific text. In the `Domain' column, CS and MS represent computer science and material science, respectively; meanwhile ML and NLP represent machine learning and natural language processing.
  }
  \label{tab:freq}
 \resizebox{\textwidth}{!}{%
  \begin{tabular}{l c c c c c}
    \toprule
    \textbf{Dataset} & \textbf{Size} & \textbf{Domain} & \textbf{Creation Method} & \textbf{\# Entity Types} & \textbf{\# Relation Types} \\
    \midrule

    \cite{gupta-manning-2011-analyzing} & 30 abstracts & NLP papers & expert & 3 & 0 \\

    ACL RD-TEC 2.0 \cite{qasemizadeh-schumann-2016-acl} & 300 abstracts & NLP papers & expert & 7 & 0 \\

   SemEval-2017 \cite{augenstein-etal-2017-semeval} & 500 paragraphs & CS, MS, Physics & student + expert & 3 & 2 \\

   SemEval-2018 \cite{gabor-etal-2018-semeval} & 500 abstracts & NLP papers & student + expert  & 0 & 6 \\

   SciERC \cite{luan-etal-2018-multi} & 500 abstracts & ML \& NLP papers & expert  & 6 & 7 \\

   NLP-TDMS \cite{hou-etal-2019-identification}  & 332 full papers & NLP papers   &  semi-auto  & 4  &  0\\ 

   SciREX \cite{jain-etal-2020-scirex} & 438 full papers  & ML conferences & semi-auto  & 4 & 0 \\

   TDMSci \cite{hou-etal-2021-tdmsci} & 2k sentences & NLP papers & expert  & 3 & 0 \\

   SciNLP-KG \cite{mondal-etal-2021-end} & 85 entities \& 625 relations & NLP papers & expert  & 3 & 4 \\

  \bottomrule
\end{tabular}
}
\end{table}


==> tables/dataset_ner_re_details.tex <==

\begin{table}

  \caption{Details of existing entity types and relation types.}
  \label{tab:freq}
 \resizebox{\textwidth}{!}{%
  \begin{tabular}{l c c c}
    \toprule
    \textbf{Dataset} & \textbf{Entity Types} & \textbf{Relation Types} & \textbf{Task Details} \\
    
    \midrule
    \cite{gupta-manning-2011-analyzing} & Focus, Technique, Domain &  - &  Key aspects extraction \\ 

    \midrule
    ACL RD-TEC 2.0 & \makecell{Method, Tool, Language Resource (LR), \\ LR Product, Model, \\ Measures and Measurements, Other} & - & Entity recognition \\  

    \midrule
   SemEval-2017 & Process, Task, Material & Hyponym-of, Synonym-of & \makecell{Mention-level keyphrase identification, \\ Mention-level keyphrase classification, \\ Mention-level semantic relation extraction} \\

    \midrule
   SemEval-2018 & -  & \makecell{Usage, Result, Model, \\ Part-whole, Topic, Comparison} & \makecell{Relation classification on clean data, \\ Relation classification on noisy data, \\ Relation extraction and classification scenario}  \\

    \midrule
    SciERC & \makecell{Task, Method, Metric,
Material, \\ Other-ScientificTerm, Generic} & \makecell{Compare, Part-of, Conjunction, \\ Evaluate-for,  Feature-of, \\ Used-for, Hyponym-of}  & \makecell{Entity recognition, \\ 
Eelation extraction, \\
Coreference resolution} \\


\midrule
NLP-TDMS & Task, Dataset, Metric, Score & - & \makecell{Task-Dataset-Metric triple classification, \\ Score extraction}   \\


\midrule
SciREX & Task, Dataset, Metric, Method & - & \makecell{Entity identification, \\ 
Predict salient entity, \\
Document level N-ary relation identification} \\


\midrule
TDMSci & Task, Dataset, Metric & - & Entity recognition \\ 

\midrule
SciNLP-KG & Task, Dataset, Metric & evaluatedOn, evaluatedBy, coreferent, and related & \makecell{Inter-entity relation extraction \\ Coreference relation extraction \\ Related relation extraction} \\

  \bottomrule
\end{tabular}
}
\end{table}


==> tables/dataset_summarization.tex <==

  \begin{tabular}{l l r c c c c c}
    \toprule
  \textbf{Year} &  \textbf{Dataset} & \textbf{Size}  &  \textbf{Type}  & \textbf{Domain} & \textbf{Creation Method} & \textbf{Single/Multiple} & \textbf{Input Information} \\
    \midrule



2014  &   TAC 2014 \cite{TAC2014}  &   10  &   Extractive  &   Biomedical  &   Automated  &   Multiple  &   Citances \\     

2014  &   CL-Summ \cite{Jaidka2014TheCL} &   10  &   Extractive  &   Computational linguistics  &   Human   &   Multiple  &   Full paper + Citances \\     

2016  &   CL-Scisumm \cite{jaidka-etal-2016-overview}  &   30  &   Extractive  &   Computational linguistics  &   Human   &   Multiple  &   Full paper + Citances \\  


2017  &   CSPubSum \cite{collins-etal-2017-supervised} &   10,000  &   Extractive  &   Computer science  &   Automated  &   Single  &   Full paper \\    

2018  &   ArXiv \cite{cohan-etal-2018-discourse}  &   215,000  &   Abstractive  &   Computer science  &   Automated  &   Single  &   Full paper \\     

2018  &   PubMed \cite{cohan-etal-2018-discourse}  &   133,000  &   Abstractive  &   Biomedical   &   Automated  &   Single  &   Full paper \\     

2019  &   PMC-SA \cite{gidiotis2019structured}  &   713,000  &   Abstractive  &   Biomedical   &   Automated  &   Single  &   Full paper \\   

2019  &   ScisummNet \cite{yasunaga_scisumm}  &   1,000  &   Extractive  &   Computational linguistics  &   Human   &   Multiple  &   Abstracts \\    

2020  &   Multi-XScience \cite{lu-etal-2020-multi-xscience}  &   40,000  &   Abstractive  &   Computer science  &   Automated  &   Multiple  &   Abstracts \\    

2021  &   SumPubMed \cite{gupta-etal-2021-sumpubmed}  &   33,000  &   Abstractive  &   Biomedical  &   Automated  &   Single  &   Full paper \\    

2022  &   MuP \cite{cohan-etal-2022-overview-first}  &   10,000  &   Abstractive  &   Computer science  &   Automated  &   Single  &   Full paper \\    

2022  &   PeerSum \cite{li-etal-2023-summarizing} &   11,000  &   Abstractive  &   Multiple domain  &   Automated  &   Multiple  &   Reviews \\     




  \bottomrule
\end{tabular}






==> tables/existing_task_dataset.tex <==
\begin{table}

  \caption{Existing tasks in scientific articles. 
  }
  \label{existing_task_dataset}
 % \resizebox{\textwidth}{!}{%
  \begin{tabular}{l l}
    \toprule
  \textbf{Grouped Name} &  \textbf{Task Details}  \\
    \midrule


\multirow{11}{3cm}{Scientific Text Acquisition}  &  \textit{Knowledge Graph Construction} \\

  & Named entity recognition \\

  & Relation extraction \\

  & Named entity disambiguation \\
  &  Coreference resolution \\
  &  Entity linking \\ 
 & ... \\ 
\cmidrule{2-2}
 & \textit{Scientific Research Dataset} \\ 
 
 & Analyzing the research data \\ 
 & Science research corpus \\ 
 & Workflow scientific mining \\ 

 \midrule
\multirow{18}{3cm}{Scientific Text Application}  &  \textit{Text Understanding} \\

  & Scientific verification \\

  & Natural language inference \\
  & Document classification \\
  & Document analysis \\
  & Semantic search \\
  & Citation recommendation \\
  & Paper evaluation \\
  & Human assistant in writing \\
  & Scientific reviewing \\
 & ... \\ 
\cmidrule{2-2}


 & \textit{Text Generation} \\ 
 & Automatic related work generation \\ 
 & Automated evidence synthesis \\ 
 & Citation text generation \\ 

 \cmidrule{2-2}
 & \textit{Text Understanding \& Generation} \\  
 & Question answering \\ 
 & Summarization \\ 


 
  \bottomrule
\end{tabular}
% }
\end{table}


==> tables/scilms_arch_size.tex <==

      \begin{tabular}{l l}
    
    \toprule
    \textbf{Types of Architecture} &  \textbf{\#} \\     \midrule
           En-only & 91 \\ 
       

        De-only & 9 \\
        Others   & 9 \\
         En-De & 8 \\ \bottomrule
    
    \end{tabular}

	\end{minipage}\hfill
	\begin{minipage}{0.6\linewidth}
		\centering
		% \captionof{figure}{Caption_2}
            \caption{Number of SciLMs modeled for each size. \label{table_summary_size}
            }
		% \label{figu:re}
		\includegraphics[width=0.8\textwidth]{images/Model-Size-Distribution.pdf}
	\end{minipage}










==> tables/scilms_domain_lang.tex <==
\begin{table}[!htb]
\parbox{.35\linewidth}{
 
  % \centering
  \caption{Distribution of SciLMs across different domains. \label{table_summary_domain}}

  \begin{tabular}{l l}

\toprule
\textbf{Domain} &  \textbf{\#} \\     \midrule
    Biomedical & 85 \\
    Chemical & 13 \\
    Multi-domain & 11 \\
    Cybersecurity & 2 \\
    Math & 2 \\
    Climate & 1 \\
    Computer Science & 1 \\
    Geoscience & 1 \\
    Manufaturing & 1 \\
    Protein & 1 \\   
    Science Education & 1 \\
    Social Science & 1 \\
    \bottomrule
\end{tabular}
}
\parbox{.6\linewidth}
{
   
    % \centering
    \caption{Distribution of SciLMs across different languages.  \label{table_summary_multilingual}
      }
      
\begin{tabular}{l l l}
    \toprule
\textbf{Language} &  \textbf{\#} & \textbf{Model Names}\\     \midrule

    Dutch & 1  & MedRoBERTa.nl \\
    Korean & 1 & KM-BERT \\ 
    Persian & 1 & SINA-BERT \\
    Turkish & 2 & Bioberturk, TurkRadBERT \\ 
    Vietnamese & 2 & ViHealthBERT, ViPubmedT5 
    \\

    French & 3 & AliBERT, DrBERT, CamemBERT-bio \\
    Japanese & 3 & ouBioBERT, UTH-BERT, AcademicRoBERTa  \\
    Spanish & 3 & Bio-cli, bsc-bio-ehr-es, EriBERTa \\

    Chinese &  4 & MC-BERT, CSL-T5, SMedBERT, ClinicalGPT \\ 

    % French & 3 & \makecell[l]{AliBERT, DrBERT, \\ CamemBERT-bio} \\
    % Japanese & 3 & \makecell[l]{ouBioBERT, UTH-BERT, \\ AcademicRoBERTa}  \\
    % Spanish & 3 & \makecell[l]{Bio-cli, EriBERTa, \\ bsc-bio-ehr-es} \\

    % Chinese &  4 & \makecell[l]{MC-BERT, CSL-T5, \\ SMedBERT, \\ ClinicalGPT} \\ 

    \midrule
    
    English   &  97   & \makecell[l]{The remaining models \\ in Tables \ref{table_lms_1}, \ref{table_lms_2} and \ref{table_lms_3}}  \\
    \bottomrule
    \end{tabular}
  }   
% \parbox{.6\linewidth}
% {
% 	\begin{minipage}{1\linewidth}
% 		\centering
% 		% \captionof{figure}{Caption_2}
%             \caption{Number of SciLMs modeled for each size. \label{table_summary_size}
%             }
% 		% \label{figu:re}
% 		\includegraphics[width=0.8\textwidth]{images/Model-Size-Distribution.pdf}
% 	\end{minipage}
%  } 
  
\end{table}






==> tables/scilms_longtable.tex <==
% \noindent\hrulefill 

{\tiny \tabcolsep=2.2pt
\begin{longtable}{l l l c c c c c c }

%   \caption{
%   Existing LMs for scientific text. 
%   In the \textbf{Training Objective} column, 
%   \textit{MLM} denotes Masked Language Model,  
%   \textit{NSP} denotes Next Sentence Prediction, and   \textit{SOP} denotes Sentence Order Prediction.
%   In the \textbf{Type of Pre-training} column, \textit{CP} and \textit{FS} denote Continual Pretraining and From Scratch, respectively. 
%  In the \textbf{Domain} column,  \textbf{CS} represents computer science, \textbf{Bio} represents Biomedical domain, \textbf{Chem} represents Chemical domain, and \textbf{Multi} represents multiple domains. 
% It is noted that the date information is chosen from the first date the paper appears on the Internet.
%   }
%   \label{table_lms_1} 


\caption{A sample long table.} 

\label{table_full_lms} \\



    \toprule
  \textbf{No.} &  \textbf{Date} & \textbf{Model} & \textbf{Architecture} &  \textbf{Training Objective} & \makecell{\textbf{Type of} \\ \textbf{Pre-training} } & \makecell{\textbf{Model} \\ \textbf{Size}} & \textbf{Domain} &  \textbf{Pre-training Corpus}  \\ \midrule

\endfirsthead

\multicolumn{9}{c}%
{{\bfseries \tablename\ \thetable{} -- continued from previous page}} \\

    \toprule
  \textbf{No.} &  \textbf{Date} & \textbf{Model} & \textbf{Architecture} &  \textbf{Training Objective} & \makecell{\textbf{Type of} \\ \textbf{Pre-training} } & \makecell{\textbf{Model} \\ \textbf{Size}} & \textbf{Domain} &  \textbf{Pre-training Corpus}  \\ \midrule
\endhead

 \midrule \multicolumn{9}{|r|}{{Continued on next page}} \\  \midrule
\endfoot


  
    
 1 &   2019/01 & BioBERT \cite{lee2020biobert} &  BERT & MLM, NSP & CP & 110M & Bio & PubMed \\ \midrule
 
    
2  &   2019/02 & BERT-MIMIC \cite{10.1093/jamia/ocz096} &  BERT & MLM, NSP & CP & \makecell{110M \& 340M} & Bio & MIMIC-III  \\ \midrule

    
3  &   2019/03 & SciBERT \cite{beltagy-etal-2019-scibert}  & BERT & MLM, NSP & CP \& FS & 110M & CS + Bio & Semantic Scholar Corpus \\ \midrule

    
4  &   2019/04 & BioELMo \cite{jin-etal-2019-probing}  & ELMo & Bi-LM & FS & 93.6M & Bio & PubMed  \\ \midrule


5   &   2019/04 & Clinical BERT (Emily)  \cite{alsentzer-etal-2019-publicly} & BERT & MLM, NSP & CP & 110M & Bio & MIMIC-III \\ \midrule


6    &   2019/04 & ClinicalBERT (Kexin) \cite{Huang2019ClinicalBERTMC}  & BERT & MLM, NSP & CP & 110M & Bio & MIMIC-III  \\ \midrule

    
7  &   2019/06 & BlueBERT \cite{peng-etal-2019-transfer}  & BERT & MLM, NSP & CP & \makecell{110M \& 340M} & Bio & PubMed + MIMIC-III \\  \midrule


8 &    2019/06 & G-BERT \cite{ijcai2019p0825} & \makecell{GNN \\ + BERT} & \makecell{Self-Prediction, \\ Dual-Prediction} & CP & 3M & Bio & MIMIC-III \\ \midrule


9 &    2019/07 & BEHRT \cite{7801}  & BERT & MLM, NSP & CP & N/A & Bio & \makecell{Clinical Practice Research Datalink}  \\ 
\midrule

    
10 &    2019/08 & BioFLAIR \cite{sharma2019bioflair}  & Flair & Bi-LM & CP & N/A & Bio & PubMed \\ \midrule
    
11 &   2019/09 & EhrBERT \cite{info:doi/10.2196/14830}  & BERT & MLM, NSP & CP & 110M & Bio & Electronic Health Record Notes \\  \midrule


12 &   2019/11 & S2ORC-SciBERT \cite{lo-etal-2020-s2orc}  & BERT & MLM, NSP & FS & 110M & Multi  & S2ORC \\ \midrule

    
13 &   2019/12 & Clinical XLNet \cite{huang-etal-2020-clinical}  & XLNet & \makecell{Generalized Autoregressive \\ Pretraining}  & CP & 110M & Bio & MIMIC-III \\ \midrule


14 &   2020/02 & SciGPT2 \cite{luu-etal-2021-explaining}  & GPT2 & LM & CP & 124M & CS &  S2ORC \\ \midrule


15 &   2020/03 & NukeBERT \cite{jain2020nukebert}  &  BERT & MLM, NSP  & CP & 110M & Chem & NText \\ \midrule



16 &   2020/04 & GreenBioBERT \cite{poerner-etal-2020-inexpensive}  & BERT & \makecell{CBOW Word2Vec, \\ Word Vector Space Alignment} & CP & 110M & Bio & PubMed + PMC \\  \midrule


17 &   2020/04 & SPECTER \cite{cohan-etal-2020-specter} & BERT & Triple-Loss & CP & 110M  & Multi &  Semantic Scholar Corpus \\ \midrule


18 & 2020/05  & BERT-XML \cite{zhang2020bertxml} & BERT  & MLM, NSP &  FS  & N/A & Bio & Electronic Health Record Notes \\ \midrule


19 &  2020/05 &	Bio-ELECTRA \cite{ozyurt-2020-effectiveness}  & ELECTRA & Replaced Token Prediction & FS & 14M & Bio & PubMed + PMC \\  \midrule

 
20 &   2020/05 & Med-BERT \cite{Rasmy2020MedBERTPC}  & BERT & \makecell{MLM, \\ Prolonged LOS Prediction}  & FS & 110M & Bio & Cerner Health Facts (Version 2017)  \\ \midrule
    


21 &   2020/05 & ouBioBERT \cite{2005.07202}  & BERT & MLM, NSP & FS & 110M & Bio & PubMed \\ \midrule



22 & 2020/07  & PubMedBERT \cite{10.1145/3458754} & BERT & \makecell{MLM,  NSP, \\ Whole-Word Masking} & FS   & 110M & Bio & PubMed \\ \midrule



23 & 2020/08  & MC-BERT \cite{zhang2020conceptualized}  &  BERT & MLM, NSP &  CP  & \makecell{110M \& 340M} & Bio & \makecell{Chinese Biomedical Community QA \\ + Chinese Medical Encyclopedia \\ + Chinese Electric Medical Record} \\ \midrule



24 & 2020/09  & BioALBERT \cite{article_naseem}  & ALBERT & MLM, SOP   &  CP  & \makecell{12M \& 18M} & Bio & PubMed + PMC \\ \midrule


25 & 2020/09  & BRLTM \cite{9369833}  & BERT  & MLM &    FS  & N/A & Bio & Private Electronic Health Record \\ \midrule


26 &  2020/10 & BioMegatron \cite{shin-etal-2020-biomegatron} &  Megatron & MLM, NSP &  CP \& FS  & \makecell{345M \& \\  800M \& 1.2B} & Bio & PubMed + PMC \\ \midrule


27  &    2020/10  &    CharacterBERT \cite{el-boukkouri-etal-2020-characterbert} &   BERT + Character-CNN & MLM, NSP & FS & 105M & Bio & MIMIC-III  + PubMed \\ \midrule


28 & 2020/10  & ChemBERTa \cite{chithrananda2020chemberta}  & RoBERTa & MLM &  FS  & 125M & Chem & SMILES from PubCHEM \\ \midrule



29 &  2020/10 & ClinicalTransformer \cite{10.1093/jamia/ocaa189}  & \makecell{BERT \\ ALBERT \\ RoBERTa \\ ELECTRA} & \makecell{MLM, NSP \\ 
MLM, SOP \\
MLM \\
Replaced Token Prediction} & CP   & \makecell{110M \\ 
12M \\
125M \\
110M} & Bio &  MIMIC-III \\ \midrule

30 & 2020/10  & SapBERT \cite{liu-etal-2021-self}  & BERT & Multi-Similarity Loss &  CP  & 110M &  Bio &   UMLS  \\  \midrule




31 & 2020/10  & UmlsBERT \cite{michalopoulos-etal-2021-umlsbert}  & BERT  &  MLM &  CP  & 110M &  Bio & MIMIC-III  \\ \midrule



32  &    2020/11  &   bert-for-radiology \cite{10.1093/bioinformatics/btaa668}  &    BERT & MLM, NSP & CP \& FS &  110M & Bio & Chest Radiograph Reports \\  \midrule


33 &    2020/11 & Bio-LM \cite{lewis-etal-2020-pretrained}  & RoBERTa & MLM & FS & \makecell{125M \& 355M} & Bio & PubMed + PMC + MIMIC-III \\ \midrule



 34 &    2020/11  &    CODER \cite{yuan2021coder}  &   \makecell{PubMedBERT \\ 
mBERT} & Contrastive Learning & CP & \makecell{110M \\ 110M} & Bio & UMLS \\ \midrule

 


35  &    2020/11  &    exBERT \cite{tai-etal-2020-exbert}   & BERT & MLM, NSP  & CP & N/A & Bio & ClinicalKey + PMC  \\ \midrule


36  &    2020/12  &    BioMedBERT \cite{chakraborty-etal-2020-biomedbert}   &    BERT & MLM, NSP & CP \& FS & 340M & Bio & BREATHE Dataset v1.0 \\  \midrule



37  &    2020/12  &    LBERT \cite{article_warikoo}  &  BERT & MLM, NSP & CP & 110M & Bio & PubMed  \\   \midrule





38  &    2021/03  &    OAG-BERT \cite{10.1145/3534678.3539210}   & BERT & MLM & FS & 110M & Multi & AMiner + PubMed    \\ \midrule




39  &    2021/04  &    CovidBERT \cite{Hebbar_Xie_2021} &    BERT & MLM, NSP & CP & 110M & Bio & Covid-19 Related Corpora \\ \midrule




40  &    2021/04  &    ELECTRAMed \cite{miolo2021electramed}   &    ELECTRA  & Replaced Token Prediction & FS & N/A & Bio & PubMed \\ \midrule

  


41  &    2021/04  &    KeBioLM  \cite{yuan-etal-2021-improving}   &    PubMedBERT & \makecell{MLM, Entity Detection, \\ Entity Linking} & CP & 110M & Bio & \makecell{Pubmed Docs \\ from PubMedDS} \\ 


   \midrule
42  &    2021/04  &    SINA-BERT \cite{taghizadeh2021sinabert}&  BERT & MLM & CP & 110M & Bio & \makecell{Manually Collected \\ (2.8M Documents)}   \\  



\midrule
43  &    2021/05  &  MathBERT (Peng) \cite{peng2021mathbert}   &   BERT  & \makecell{MLM, Masked Substructure Prediction, \\ Context Correspondence Prediction} & CP & 110M & Math & \makecell{Formula-Context Pairs \\ Extracted from arXiv} \\ \midrule


44  &    2021/05  &   NukeLM \cite{burke2021nukelm}   & \makecell{BERT \\ RoBERTa-Base \\ RoBERTa-Large} & MLM & CP & \makecell{110M \\ 125M \\  355M} & Chem & \makecell{U. S. Department of \\ Energy Office Scientific and \\ 
Technical Information Database} \\ \midrule 


45  &    2021/05  &    ProteinBERT \cite{10.1093/bioinformatics/btac020} &  BERT &  Corrupted Token, Annotation Prediction & FS & 16M & Bio & UniProtKB/UniRef90 + GO \\ \midrule


46 &    2021/05  &    SciFive  \cite{phan2021scifive}   & T5 & Span Corruption Prediction  & CP & \makecell{220M  \\ \&  770M} & Bio & PubMed + PMC \\ \midrule


47  &    2021/06  &    BioELECTRA \cite{kanakarajan-etal-2021-bioelectra}  &   ELECTRA & Replaced Token Prediction & CP \& FS & 110M & Bio & PubMed + PMC \\ \midrule


48  &    2021/06  &    ChemBERT \cite{doi:10.1021/acs.jcim.1c00284}  &  RoBERTa & MLM & CP & 110M  & Chem & 
ACS Publications \\ \midrule 


49  &    2021/06  &    EntityBERT \cite{lin-etal-2021-entitybert}  & BERT  & Entity-Centric MLM & CP & 110M   & Bio & MIMIC \\ \midrule 



50  &    2021/06  & MathBERT (Shen) \cite{shen2023mathbert} & RoBERTa & MLM &  CP & 110M & Math & \makecell{Mathematics Curricula \\  + Mathematics Textbooks \\ + Mathematics Course Syllabi \\ + Mathematics Paper Abstracts} \\ \midrule


  
51  &    2021/07  &    MedGPT  \cite{kraljevic2021medgpt}  &  \makecell{GPT2 + GLU \\ + RotaryEmbed}  & LM & CP & N/A & Bio &  Electronic Health Record Notes \\ \midrule 


52  &    2021/08  &    SMedBERT  \cite{zhang2021smedbert}  & SMedBERT & \makecell{Masked Neighbor Modeling, SOP, \\
Masked Mention Modeling, MLM} & FS & N/A & Bio & DXY BBS (Bulletin Board System)  \\ \midrule 




53  &    2021/09  &  Bio-cli \cite{carrino2021biomedical} & RoBERTa & \makecell{MLM, Subword Masking \\ or Whole Word Masking} & FS & 125M & Bio & Clinical Corpus + Biomedical Corpus \\ \midrule 





54  &    2021/09  &    MatSciBERT \cite{gupta2022matscibert}  &  BERT & MLM & CP & 110M & Chem & Material Science Corpus \\ \midrule 


55  &    2021/10  &    ClimateBert  \cite{webersinke2022climatebert}  & DistilROBERTA & MLM & CP & 66M & Climate & \makecell{News Articles  + Research Abstracts \\ + Corporate Climate Reports} \\ \midrule 





  
56  &    2021/10  &    MatBERT \cite{Trewartha2022-sl}  &  BERT & MLM & FS & 110M & Chem &  \makecell{Peer-Reviewed Materials \\ Science Journal Articles} \\ \midrule 



 



57  &    2021/11  &   UTH-BERT \cite{aclinical_kawazoe}    & BERT & MLM, NSP & FS & 110M & Bio & \makecell{Clinical Texts from The \\ University of Tokyo Hospital}   \\ \midrule 



58  &    2021/12  &    ChestXRayBERT \cite{9638337}   &  BERT & MLM, NSP & CP & 110M & Bio & 20617 Scientific Papers in PMC  \\ \midrule 
% Chest Radiology





59  &    2021/12  &    MedRoBERTa.nl \cite{Verkijk_Vossen_2021}  &   RoBERTa & MLM & FS & 123M & Bio & \makecell{Dutch Hospital Notes, from EHRs} \\ \midrule 



60  &    2021/12  &    PubMedELECTRA \cite{TINN2023100729}   &   ELECTRA & Replaced Token Prediction & FS & \makecell{110M \\ \& 335M} & Bio & PubMed  \\ \midrule 



% 61  &    2022/01  &    \makecell[l]{Clinical-BigBird \\ Clinical-Longformer} \cite{li2022clinicallongformer}  & En &  \makecell{BigBird \\ Longformer}  & MLM & CP & \makecell{166M \\ 149M}  & Bio & MIMIC-III  \\ \midrule 
61  &    2022/01  &   Clinical-Longformer  \cite{li2022clinicallongformer}   &  \makecell{BigBird \\ Longformer}  & MLM & CP & \makecell{166M \\ 149M}  & Bio & MIMIC-III  \\ \midrule 
  
  
62 &    2022/03 & BioLinkBERT \cite{yasunaga-etal-2022-linkbert}   & BERT & \makecell{MLM, \\ Document Relation Prediction}  & FS & \makecell{110M \\ \& 340M} & Bio  & PubMed + PMC \\  \midrule 
 



63  &    2022/04  &    BioBART  \cite{yuan-etal-2022-biobart}   &  BART  & \makecell{Text Infilling,\\ Sentence Permutation} & CP & \makecell{140M \\ \& 400M} & Bio & PubMed  \\ \midrule 



  
64  &    2022/04  &    SecureBERT  \cite{1a3e2a1ca6f94c7589c870bc0b3e1e31}   & RoBERTa & MLM & CP & 125M & Cybersecurity & \makecell{Manually Collected \\ (98,411 Documents)}   \\ \midrule 



65   &    2022/05  &    BatteryBERT \cite{doi:10.1021/acs.jcim.2c00035}   &  BERT & MLM & CP \& FS & 110M & Chem & \makecell{Battery-Related Scientific Papers \\ from RSC, Elsevier, Springer} \\ \midrule 




66  &    2022/05  &   bsc-bio-ehr-es  \cite{carrino-etal-2022-pretrained}   &  RoBERTa & MLM & FS & 125M & Bio & \makecell{Electronic Health Record Corpus
\\ + Biomedical Corpus} \\ \midrule 


67   &    2022/05  &    ChemGPT  \cite{frey2022neural}  & GPT & Autoregressive LM & FS & 1B & Chem & SMILES from PubCHEM \\ \midrule 


68  &    2022/05  &    PathologyBERT \cite{santos2022pathologybert}    &  BERT & MLM, NSP & FS & 110M & Bio &  \makecell{Manually Labeled Pathology Reports \\
+ Unlabeled Pathology Reports from EUH} \\ \midrule 





69  &    2022/05  &    ScholarBERT \cite{hong2023diminishing}   & BERT &  MLM & FS & 770M & Multi & Public Resource Dataset \\ \midrule 



  
70 &    2022/06 & RadBERT \cite{yan2022radbert}   & RoBERTa & MLM & CP & 110M & Bio &  Radiology Reports \\ \midrule



71  &    2022/06  &    SciDeBERTa \cite{jeong2022scideberta}   &  DeBERTa &  MLM & CP & N/A & Multi & S2ORC \\  \midrule 
  

72  &    2022/06  &    SsciBERT \cite{10.1007/s11192-022-04602-4} & BERT & MLM, NSP & CP & 110M & Social Science  & Collected from Web of Science \\  \midrule



73 &    2022/06 & ViHealthBERT \cite{minh-etal-2022-vihealthbert}  & PhoBERT & \makecell{MLM, NSP, \\ Capitalized Prediction} & CP & 110M & Bio & \makecell{OSCAR Dataset \\ + Their Text Mining Corpus} \\  \midrule 




74  &    2022/07  &    Clinical Flair \cite{rojas-etal-2022-clinical}   &  \makecell{Flair} & Character-Level Bi-LM & CP & N/A & Bio & Free-Text Diagnostic Suspicions \\  \midrule 


75  &    2022/08  &    KM-BERT  \cite{Kim2022-er}  &  BERT & MLM, NSP & CP & 99M & Bio &  \makecell{Medical Textbooks \\ + Health Information News \\ + Medical Research Articles}  \\ \midrule





76  &    2022/08  &    MaterialsBERT (Shetty) \cite{Shetty_2023}   &  PubMedBERT & MLM, NSP, Whole-Word Masking & CP & 110M & Chem &  Polymer Scholar  \\ \midrule 


77   &    2022/08  &    ProcessBERT \cite{KATO2022957}   &  
 BERT & MLM, NSP & CP & 110M & Chem & ChemECorpus  \\ \midrule 



78 &    2022/09 & BioGPT \cite{10.1093/bib/bbac409}   & GPT & Autogressive LM & FS & \makecell{347M  \\ \& 1.5B} & Bio & PubMed \\ \midrule



79  &    2022/09  &    ChemBERTa-2 \cite{ahmad2022chemberta}  &  RoBERTa &  MLM, Multi-Task Regression & FS & 125M & Chem & SMILES from PubCHEM   \\  


 \midrule
80  &    2022/09  & CSL-T5   \cite{li-etal-2022-csl}   &   T5 & \makecell{Fill-in-the-blank-style \\ Denoising Objective} & FS & 220M & Multi & Chinese Academic Journals \\ 


 \midrule 
81  &    2022/09  &    MaterialBERT (Yoshitake) \cite{yoshitake2022materialbert}  &  BERT & MLM, NSP & FS & 110M &  Chem & Scientific Articles from NIMS \\  



\midrule
82  &    2022/10  & AcademicRoBERTa \cite{yamauchi-etal-2022-japanese} & RoBERTa & MLM & FS & 125M & Multi & CiNii Articles \\  


\midrule
 83  &    2022/10  & Bioberturk \cite{PPR:PPR560833}  & BERT & MLM, NSP & CP \& FS & N/A & Bio & \makecell{Turkish Medical Articles \\ +
Turkish Radiology Thesis} \\ 


\midrule
84  &    2022/10  &    DRAGON \cite{yasunaga2022deep}   &  GreaseLM & \makecell{MLM, KG Link Prediction} & CP & 360M & Bio & PubMed + UMLS KG \\  \midrule



85  &    2022/10  &    UCSF-BERT \cite{sushil2022developing}   &   BERT & MLM, NSP & FS & 135M & Bio &  Clinical Notes of UCSF Health  \\ \midrule 


86  &    2022/10  & ViPubmedT5 \cite{phan2023enriching}  & T5 & Spans-masking Learning & CP & 220M & Bio & ViPubmed \\ \midrule




87 &    2022/11 & Galactica \cite{taylor2022galactica}  & GPT & Autogressive LM & FS & \makecell{125M \\ \& 1.3B \& 6.7B \\ \& 30B \& 120B} & Multi &  \makecell{Papers, Reference Material, Knowledge Bases, \\Common Crawl, Code, <work> Datasets} \\ 
\midrule



  
88  &    2022/11  &    VarMAE \cite{hu-etal-2022-varmae}  &  RoBERTa & MLM & CP & 110M & Multi  & \makecell{Semantic Scholar Corpus \\ + Finance-Related Online Platforms}  \\ \midrule



89  &    2022/12  &    AliBERT \cite{berhe-etal-2023-alibert}  & BERT & MLM & FS & 110M & Bio & \makecell{Drug Database 550MB + Cochrane 27MB  + \\
 Articles 4300MB  + Thesis 300MB 
+ RCP 2200MB}  \\ \midrule


90 &    2022/12 & BioMedLM \cite{cite_BioMedLM}   & GPT2 & Autogressive LM & FS & 2.7B &  Bio  &  PubMed + PMC \\ \midrule


  
91  &    2022/12  &    BioReader \cite{frisoni-etal-2022-bioreader}  & T5 + RETRO & MLM & CP & 229.5M & Bio & PubMed  \\ \midrule




92  &    2022/12  &    ClinicalT5 \cite{lu-etal-2022-clinicalt5}  & T5 & Span-mask Denoising Objective  & CP & \makecell{220M \\ \& 770M} & Bio & MIMIC-III  \\ \midrule


93  &    2022/12   & CySecBERT \cite{bayer2022cysecbert}  & BERT & MLM, NSP & CP & 110M  & Cybersecurity & \makecell{Blog Data + arXiv Data + Twitter Data \\ + National Vulnerability Database} \\ \midrule



94  &    2022/12  &    GatorTron \cite{Yang2022-pf}  & BERT & MLM & FS & 8.9B & Bio &  \makecell{De-identified Clinical Notes \\ + PubMed + Wikipedia}  \\ \midrule



95  &    2022/12   & Med-PaLM \cite{singhal2023large}  & Flan-PaLM & Instruction Prompt Tuning & CP & 540B & Bio & N/A \\ \midrule

  
% from here

96  &    2023/01  &    Clinical-T5 \cite{Clinical_T5_lehman} &  T5   & \makecell{Fill-in-the-blank-style \\ Denoising Objective} & \makecell{CP \& FS} & \makecell{220M \\ \& 770M}  & Bio & MIMIC-III + MIMIC-IV  \\ \midrule


% 97  &    2023/01  &    \makecell[l]{CPT-BigBird \\ CPT-Longformer} \cite{Louisa_heyarticle}  & En &  \makecell{BigBird \\ Longformer}  & MLM & CP & \makecell{166M \\ 149M}  & Bio & Senior Scholars' Basket of Journals  \\ \midrule 
97  &    2023/01  &    CPT-BigBird \cite{Louisa_heyarticle}   &  \makecell{BigBird \\ Longformer}  & MLM & CP & \makecell{166M \\ 149M}  & Bio & Senior Scholars' Basket of Journals  \\ \midrule 

98  &    2023/01  &   ProtST  \cite{xu2023protst}   &  BERT   & \makecell{Masked Protein Modeling \\ + Contrastive Learning \\
+ Multi-modal Masked Prediction} & CP \& FS  &  N/A  &  Protein  &  ProtDescribe  \\ \midrule


99  &    2023/01  &  SciEdBERT   \cite{liu2023context}    &  BERT   & MLM & CP  & 110M &  Science Education &  \makecell{The Academic Journal Dataset \\ + Students’ Responses}   \\ \midrule




100  &    2023/02  &    Bioformer \cite{fang2023bioformer}  &  BERT   & MLM, NSP & FS & 43M & Bio & PubMed + PMC   \\ \midrule


101  &    2023/02  &   \makecell[l]{Lightweight  Clinical \\ Transformers \cite{rohanian2023lightweight} }  &  DistilBERT   &  \makecell{MLM, \\ Knowledge Distillation Objective} & CP  & \makecell{15M \& 18M \\ \& 25M \& 65M} & Clinical & MIMIC-III   \\ \midrule




102  &    2023/03  &    ManuBERT \cite{ManuBERT_kumar} & BERT & MLM & CP & \makecell{110M  \\ \& 126M} & Manufaturing & \makecell{Manufacturing Process Journals \\ + Six Commonly Used Textbooks}  \\ \midrule 



103  &    2023/03  &   RAMM  \cite{yuan2023ramm}   &  PubmedBERT   & \makecell{MLM, Image-Text Matching, \\ Image-Text Contrastive Learning} & CP  & N/A & Bio & ROCO, MIMIC-CXR, PMCPM   \\ \midrule



104  &    2023/04  &  DrBERT  \cite{labrak2023drbert}  &  RoBERTa & MLM & FS & 110M & Bio & \makecell{Online Sources \\ + Private Hospital Stays Reports}  \\ \midrule 


105  &    2023/04  &  MOTOR   \cite{lin2023medical}   &  BLIP   & \makecell{MLM, Image-Text Matching, \\ Image-Text Contrastive Learning} &  CP   &  N/A & Bio &   MIMIC-CXR \\ \midrule




106  &    2023/05  &   BiomedGPT \cite{zhang2023biomedgpt}  &  BART & \makecell{Text Infilling,\\ Sentence Permutation} & FS & \makecell{33M \\ \& 93M \\ \& 182M}  & Bio &  \makecell{CheXpert + PathVQA + Retinal Fundus \\ + International Skin Imaging Collaboration \\  + Peir Gross   + CytoImageNet + MIMIC-III \\ + DeepLesion + NCBI BioNLP Corpus \\ + MedICaT + PubMed + SLAKE + IU X-ray  } \\ \midrule 


107  &    2023/05  &   Patton  \cite{jin-etal-2023-patton}    &  \makecell{GNN-nested \\ Transformer}  & \makecell{Network-contextualized MLM,  \\ Masked Node Prediction} & CP  & N/A &  Multi &  \makecell{Academic Networks from Microsoft Academic Graph, \\ E-commerce Networks from Amazon}  \\ \midrule


108  &    2023/05  &  TurkRadBERT \cite{türkmen2023harnessing} & BERT & MLM, NSP & CP \& FS & 110M & Bio &  \makecell{General Turkish Corpus + Head CT Reports \\ + Turkish Biomedical Corpus \\ 
+ Turkish Electronic Radiology Theses} \\ \midrule


109  &    2023/06  &   CamemBERT-bio  \cite{touchent2023camembertbio}  & CamemBERT    & Whole Word Masking  & CP  &  111M & Bio &  Biomed-fr: ISTEX, CLEAR, and E3C  \\ \midrule



110  &    2023/06  &   ClinicalGPT \cite{wang2023clinicalgpt} & T5 & \makecell{Supervised Fine Tuning \\ 
Rank-based Training} & \newupdate{Instruction Tuning} & \newupdate{CP} & Bio & Supervised Task Datasets  \\  \midrule


% 111  &    2023/06  &   \makecell[l]{EriBERTa \\ EriBERTa-Longformer}  \cite{delaiglesia2023eriberta}  &  En &  \makecell{RoBERTa \\ Longformer}   & MLM & CP \& FS  & \makecell{125M \\ 149M} & Bio &  \makecell{MIMIC-III, EMEA, ClinicalTrials, PubMed, \\ SNOMED-CT, SPACCC,  UFAL, Wikipedia Med, \\ Private Clinical Documents, Medical Crawler}  \\ \midrule
111  &    2023/06  &   EriBERTa  \cite{delaiglesia2023eriberta}  &  \makecell{RoBERTa \\ Longformer}   & MLM & CP \& FS  & \makecell{125M \\ 149M} & Bio &  \makecell{MIMIC-III, EMEA, ClinicalTrials, PubMed, \\ SNOMED-CT, SPACCC,  UFAL, Wikipedia Med, \\ Private Clinical Documents, Medical Crawler}  \\ \midrule


112  &    2023/06  &  K2   \cite{deng2023k2}  &  LLaMA   & Cosine Loss   & CP  & 7B & Geoscience &  \makecell{Geoscience-Related Wikipedia Pages, \\ 
Open-access Geoscience Papers, \\
Geoscience Paper’s Abstracts}   \\ \midrule



113  &    2023/06  &    PharmBERT \cite{10.1093/bib/bbad226}   &  BERT   & MLM & CP  & 110M & Bio &  DailyMed  \\ \midrule

%%%%

114  &    2023/07  &    BioNART \cite{asada-miwa-2023-bionart}   &  BERT   & Connectionist Temporal Classification & CP  & 110M &  Bio &  PubMed/MEDLINE   \\ \midrule


115  &    2023/07  &    BIOptimus \cite{pavlova-makhlouf-2023-bioptimus}   &  BERT   & MLM & CP  & 110M & Bio &  PubMed   \\ \midrule




116  &    2023/07  &    KEBLM \cite{LAI2023104392}  &  BERT & \makecell{MLM, Ranking Objective, \\
Contrastive Learning}  & CP  & N/A  & Bio &   UMLS, PubChem, MSI  \\ \midrule




117  &    2023/08  &    GIT-Mol \cite{liu2023gitmol}   &  \makecell{\newupdate{BLIP2}}   & \makecell{Xmodal-Text Matching, \\ 
Xmodal-Text Contrastive Learning}  &  N/A &  700M & Chem &  PubChem \\ 





  \bottomrule
\end{longtable}
}


==> tables/scilms_results_01.tex <==

% Table result - 1
\begin{table}

  \caption{
  Tasks and Datasets are used in existing LMs for scientific text.
  The underlying datasets are those in which the proposed SciLMs outperform previous models or achieve SOTA results.
  }
  \label{tab_result_1}

      \resizebox{\textwidth}{!}{%
  \begin{tabular}{p{0.22cm}p{2.2cm}p{5.8cm}p{9.7cm}}
    \toprule
 \textbf{No.} &   \textbf{Model} & \textbf{Tasks } & \textbf{Datasets}\\



    
\midrule
\multirow{4}{0.22cm}{1} & \multirow{4}{1.6cm}{BioBERT} & \multirow{2}{4.5cm}{\textcolor{blue}{Named Entity Recognition}} & \underline{NCBI-disease}, \underline{BC5CDR-disease}, \underline{BC5CDR-chemical}, \underline{BC4CHEMD}, \underline{BC2GM}, JNLPBA, LINNAEUS,  i2b2 2010, Species-800 \\

  &  & \textcolor{purple}{Relation Extraction} & \underline{ChemProt}, GAD, EU-ADR  \\
 
&    & \textcolor{orange}{Question Answering} & \underline{BioASQ 5b-factoid}, \underline{BioASQ 6b-factoid}, BioASQ 4b-factoid \\
    



 \midrule
 \multirow{1}{0.22cm}{2} &    \multirow{1}{1.8cm}{BERT-MIMIC} &  \multirow{1}{4.5cm}{\textcolor{blue}{Named Entity Recognition}} & \underline{i2b2 2010}, \underline{i2b2 2012}, \underline{SemEval 2014 Task 7}, \underline{SemEval 2015 Task 14} \hl{(All)}  \\




 \midrule
\multirow{5}{0.3cm}{3} &    \multirow{5}{1.2cm}{SciBERT} &  \textcolor{blue}{Named Entity Recognition} &  \underline{BC5CDR}, \underline{SciERC}, JNLPBA, NCBI-disease \\

&    & \textcolor{magenta}{PICO Extraction} & \underline{EBM-NLP} \\
    
&    & \textcolor{teal}{Text Classification} & \underline{ACL-ARC}, \underline{SciCite}, Paper Field \\ 

&    & \textcolor{purple}{Relation Extraction} & \underline{ChemProt}, SciERC \\ 

&    & \textcolor{cyan}{Dependency Parsing}  & GENIA-LAS, GENIA-UAS\\




\midrule
 \multirow{2}{0.3cm}{4} &    \multirow{2}{1.2cm}{BioELMo} &  \textcolor{blue}{Named Entity Recognition} & \underline{BC2GM} (Probing task),  CoNLL 2003 \\

& & \textcolor{Bittersweet}{Natural Language Inference} & \underline{MedNLI} (Probing task), SNLI\\




\midrule
 \multirow{2}{1.6cm}{5} &    \multirow{2}{2.2cm}{Clinical BERT (E)} &  \textcolor{blue}{Named Entity Recognition} &  i2b2 2006, i2b2 2010, i2b2 2012, i2b2 2014 \\

& & \textcolor{Bittersweet}{Natural Language Inference} & \underline{MedNLI} \\




\midrule
 \multirow{1}{1.6cm}{6} &    \multirow{1}{2.2cm}{ClinicalBERT (K)} &  \multirow{1}{4.5cm}{\textcolor{black}{Readmission Prediction}} & \multirow{1}{7.4cm}{30-day hospital
readmission prediction}  \\






\midrule
 \multirow{5}{0.3cm}{7} &    \multirow{5}{1.2cm}{BlueBERT} &  \textcolor{blue}{Named Entity Recognition}  &     \underline{BC5CDR-disease}, \underline{BC5CDR-chemical}, \underline{ShARe/CLEF} \\

 & & \textcolor{purple}{Relation Extraction}  & \underline{DDI}, \underline{ChemProt}, \underline{i2b2 2010}\\ 

& & \textcolor{Green}{Sentence Similarity}  & \underline{BIOSSES}, \underline{MedSTS}\\ 

& & \textcolor{brown}{Document Multi-label Classification}  & \underline{HOC}\\ 

& & \textcolor{Bittersweet}{Natural Language Inference} &  \underline{MedNLI} \hl{(All)}\\ 




\midrule
 8 &    G-BERT &  \textcolor{Fuchsia}{Medication Recommendation Task}  &     Medication Recommendation Task \\




\midrule
9 &    BEHRT &  \textcolor{BlueViolet}{Disease Prediction}  & \underline{Next Visit}, \underline{Next 6M}, \underline{Next 12M} \hl{(All)}   \\




\midrule
10 &    BioFLAIR &  \textcolor{blue}{Named Entity Recognition}  &  \underline{BC5CDR}, \underline{Species-800}, NCBI-disease, LINNAEUS, JNLPBA, BC5CDR-disease  \\




\midrule
 \multirow{1}{0.3cm}{11} &    \multirow{1}{1.2cm}{EhrBERT} & \multirow{1}{4.5cm}{\textcolor{black}{Entity Normalization}}  & \underline{MADE 1.0}, \underline{NCBI-disease}, \underline{CDR} \hl{(All)}  \\



\midrule
\multirow{5}{0.3cm}{12} &    \multirow{5}{2.2cm}{S2ORC-SciBERT} &  \textcolor{blue}{Named Entity Recognition} &  BC5CDR, SciERC, JNLPBA, NCBI-disease \\

&    & \textcolor{magenta}{PICO Extraction} & EBM-NLP \\
    
&    & \textcolor{teal}{Text Classification} & ACL-ARC, SciCite, Paper Field \\ 

&    & \textcolor{purple}{Relation Extraction} & ChemProt, SciERC \\ 

&    & \textcolor{cyan}{Dependency Parsing}  & GENIA-LAS, GENIA-UAS\\




\midrule
 \multirow{1}{0.3cm}{13} &    \multirow{1}{2.2cm}{Clinical XLNet} &  \textcolor{black}{Prolonged Mechanical Ventilation  Prediction}   & \multirow{1}{7cm}{\underline{PMV}, \underline{Mortality} \hl{(All)}}   \\



\midrule
14  &   SciGPT2 &  \textcolor{black}{Relationship Explanation Task} &     Relationship Explanation Task \\



\midrule
15  &   NukeBERT  &  \textcolor{orange}{Question Answering} &     NQUAD \hl{(All)} \\ 



\midrule
\multirow{2}{0.3cm}{16}  &   \multirow{2}{1.8cm}{GreenBioBERT}  &  \multirow{2}{4.5cm}{\textcolor{blue}{Named Entity Recognition}} & \underline{BC5CDR-chemical}, \underline{BC4CHEMD}, \underline{Species-800},  BC5CDR-disease, NCBI-disease, BC2GM, JNLPBA, LINNAEUS   \\ 




 \midrule
 \multirow{4}{0.3cm}{17} &    \multirow{4}{1.8cm}{SPECTER} &  \textcolor{teal}{Text Classification} &  \underline{MeSH}, \underline{MAG} \\ 

 & & \textcolor{NavyBlue}{Citation Prediction} &  \underline{Co-Cite}, Cite \\ 

 & & \textcolor{RubineRed}{User Activity Prediction} & \underline{Co-Views}, \underline{Co-Reads} \\ 

& &  \textcolor{Fuchsia}{Paper Recommendation Task} &  \underline{Paper Recommendation Task} \\ 



\midrule
18  &   BERT-XML  &  \textcolor{black}{ICD Classification} &  \underline{ICD Classification}  \hl{All} \\ 




\midrule
\multirow{3}{0.22cm}{19} & \multirow{3}{2.3cm}{Bio-ELECTRA} & \textcolor{blue}{Named Entity Recognition} & BC2GM, BC4CHEMD, NCBI-disease, LINNAEUS \\

  &  & \textcolor{purple}{Relation Extraction} & GAD, ChemProt  \\
 
&    & \textcolor{orange}{Question Answering} & \underline{BioASQ 8b-yes/no}, \underline{BioASQ 5b based}, BioASQ 8b-factoid \\





\midrule
 \multirow{2}{0.3cm}{20} &    \multirow{2}{1.6cm}{Med-BERT} &  \multirow{2}{4.5cm}{\textcolor{BlueViolet}{Disease Prediction}}  &  \underline{Heart failure in diabetes patients} (DHF-Cerner), \underline{Pancreatic cancer} (PaCa-Cerner, PaCa-Truven) \hl{(All)}   \\




\midrule
 \multirow{5}{0.3cm}{21} &    \multirow{5}{1.6cm}{ouBioBERT} &  \textcolor{blue}{Named Entity Recognition}  &     \underline{BC5CDR-disease}, BC5CDR-chemical, ShARe/CLEF \\

 & & \textcolor{purple}{Relation Extraction}  & \underline{DDI}, \underline{ChemProt}, i2b2 2010\\ 

& & \textcolor{Green}{Sentence Similarity}  & \underline{BIOSSES}, MedSTS\\ 

& & \textcolor{brown}{Document Multi-label Classification}  & HOC \\ 

& & \textcolor{Bittersweet}{Natural Language Inference} &  MedNLI \\ 








  \bottomrule
\end{tabular}
}

\end{table}



==> tables/scilms_results_02.tex <==
% Table result - 2
\begin{table}

  \caption{
  A continuation of the table from Table \ref{tab_result_1}.
  Tasks and Datasets are used in existing LMs for scientific text.
  The underlying datasets are those in which the proposed SciLMs outperform previous models or achieve SOTA results.
  }
  \label{tab_result_2}

\resizebox{\textwidth}{!}{%
  \begin{tabular}{p{0.22cm}p{2.3cm}p{4.6cm}p{9.2cm}}
    \toprule
 \textbf{No.} &   \textbf{Model} & \textbf{Tasks } & \textbf{Datasets}\\











\midrule
 \multirow{6}{0.3cm}{22} &    \multirow{6}{1.8cm}{PubMedBERT} &  \textcolor{blue}{Named Entity Recognition} &  \underline{BC5CDR-disease}, \underline{BC5CDR-chemical}, \underline{JNLPBA}, \underline{BC2GM}, NCBI-disease  \\

  & & \textcolor{purple}{Relation Extraction} & \underline{ChemProt}, \underline{DDI}, \underline{GAD} \\ 

& & \textcolor{magenta}{PICO Extraction} &  \underline{EBM PICO}\\

& & \textcolor{Green}{Sentence Similarity} & \underline{BIOSSES} \\

& & \textcolor{brown}{Document Multi-label Classification}  & \underline{HOC} \\

& & \textcolor{orange}{Question Answering}  & \underline{BioASQ}, PubMedQA \\





\midrule
 \multirow{6}{0.3cm}{23} &    \multirow{6}{1.8cm}{MC-BERT} &  \textcolor{blue}{Named Entity Recognition} &  \underline{cEHRNER}, \underline{cMedQANER}  \\

& & \textcolor{orange}{Question Answering}  & \underline{cMedQNLI}, \underline{cMeQA}\\

&    & \textcolor{teal}{Text Classification} & \underline{cMedTC} \\ 

& & \textcolor{black}{Intent Classification} &  \underline{cMedIC}\\

& & \textcolor{black}{Paraphrase Identification} & \underline{cMedQQ} \\

& & \textcolor{RawSienna}{Information Retrieval}  & \underline{cMedIR} \hl{(All)} \\




\midrule
\multirow{7}{0.3cm}{24}  &   \multirow{7}{1.8cm}{BioALBERT}  &  \multirow{2}{4.5cm}{\textcolor{blue}{Named Entity Recognition}} &  \underline{NCBI-disease}, \underline{BC5CDR}, \underline{BC4CHEMD}, \underline{BC2GM}, \underline{JNLPBA}, \underline{LNNAEUS}, \underline{Species-800}, \underline{Share/Clefe} \\ 


  & & \textcolor{purple}{Relation Extraction} & \underline{ChemProt}, \underline{DDI}, \underline{i2b2}, GAD, Euadr \\ 

& & \textcolor{Green}{Sentence Similarity} & \underline{BIOSSES}, \underline{MedSTS} \\

& & \textcolor{brown}{Document Multi-label Classification}  & \underline{HOC} \\

& & \textcolor{orange}{Question Answering}  & \underline{BioASQ} \\

 & & \textcolor{Bittersweet}{Natural Language Inference} & MedNLI \\









\midrule
25  &   BRLTM  &  \textcolor{black}{Depression Prediction} &  \underline{Depression Prediction}  \hl{(All)} \\ 





\midrule
\multirow{3}{0.22cm}{26} & \multirow{3}{1.6cm}{BioMegatron} & \textcolor{blue}{Named Entity Recognition} &  \underline{BC5CDR-chemical}, \underline{BC5CDR-disease}, \underline{NCBI-disease} \\

  &  & \textcolor{purple}{Relation Extraction} &  \underline{ChemProt} \\
 
&    & \textcolor{orange}{Question Answering} & \underline{BioASQ 7b-factoid} \hl{(All)} \\





\midrule
 \multirow{4}{0.3cm}{27} &    \multirow{4}{1.8cm}{CharacterBERT} &  \textcolor{blue}{Named Entity Recognition}  &   \underline{i2b2 2010}   \\

 & & \textcolor{purple}{Relation Extraction}  & \underline{DDI}, \underline{ChemProt} \\ 

& & \textcolor{Green}{Sentence Similarity}  & ClinicalSTS \\ 

& & \textcolor{Bittersweet}{Natural Language Inference} &  \underline{MedNLI} \\ 




\midrule
28  &   ChemBERTa & MoleculeNet Task  &  BBBP, ClinTox, HIV, Tox21  \\ 





\midrule
29  &   ClinicalTransformer  &  \textcolor{blue}{Named Entity Recognition} & \underline{i2b2 2010}, \underline{i2b2 2012}, \underline{n2c2 2018}  \hl{(All)}  \\ 





\midrule
\multirow{2}{0.3cm}{30}  &   \multirow{2}{1.8cm}{SapBERT}  &  \multirow{2}{4.5cm}{\textcolor{Apricot}{Entity Linking}} & \underline{NCBI-disease}, \underline{BC5CDR-disease}, \underline{BC5CDR-chemical}, \underline{MedMentions}, \underline{AskAPatient}, \underline{COMETA}  \hl{(All)} \\ 





\midrule
\multirow{3}{0.22cm}{31} & \multirow{3}{1.6cm}{UmlsBERT} & \textcolor{blue}{Named Entity Recognition} &  \underline{i2b2 2010}, \underline{i2b2 2012} \\

 & & \textcolor{Bittersweet}{Natural Language Inference} & \underline{MedNLI} \\
 
 & & \textcolor{SeaGreen}{De-Identification} & \underline{i2b2 2006}, i2b2 2014 \\ 





\midrule
 \multirow{1}{0.3cm}{32} &    \multirow{1}{2.8cm}{bert-for-radiology} &  \textcolor{teal}{Text Classification}  &   \underline{Binary Classifier}, \underline{Classification of CT Reports}, Multi-label Classification  \\

%  & & Multi-label Classification  & Multi-label Classification \\ 

% &    & Classification of CT Reports & \underline{Classification of CT Reports} (\textit{RAD-BERT version}) \\ 





\midrule
 \multirow{6}{0.3cm}{33} &    \multirow{6}{1.2cm}{Bio-LM} &  \multirow{2}{4cm}{\textcolor{blue}{Named Entity Recognition}} & \underline{BC5CDR-chemical}, \underline{BC5CDR-disease}, \underline{JNLPBA}, \underline{NCBI-disease}, \underline{BC4CHEMD}, \underline{BC2GM}, \underline{LINNAEUS}, \underline{Species-800}, \underline{i2b2-2010}, \underline{i2b2-2012}  \\

 & & \textcolor{purple}{Relation Extraction} & \underline{ChemProt}, \underline{DDI}, \underline{i2b2 2010}, GAD, EU-ADR \\ 

 & & \textcolor{SeaGreen}{De-Identification} & \underline{i2b2 2014} \\ 
 
 & & \textcolor{brown}{Document Multi-label Classification}  & HOC\\
 & & \textcolor{Bittersweet}{Natural Language Inference} & \underline{MedNLI} \\




\midrule
 \multirow{3}{0.3cm}{34} &    \multirow{3}{1.8cm}{CODER} &  \textcolor{black}{Term Normalization}  &   \underline{Cadec}, \underline{PsyTar}, MANTRA  \\

 & & \textcolor{black}{Medical Embeddings}  & \underline{MCSM} \\ 

&    & \textcolor{purple}{Relation Extraction} & \underline{DDBRC} (\textit{CODER-Eng version}) \\ 







\midrule
 \multirow{2}{0.3cm}{35} &    \multirow{2}{1.2cm}{exBERT} &  \textcolor{blue}{Named Entity Recognition} & \underline{MTL-Bioinformatics-2016}  \\

  & & \textcolor{purple}{Relation Extraction} & \underline{MTL-Bioinformatics-2016}  \hl{(All)} \\ 








  \bottomrule
\end{tabular}
}

\end{table}



==> tables/scilms_results_03.tex <==




% Table result - 3
\begin{table}

  \caption{
  A continuation of the table from Tables \ref{tab_result_1} and \ref{tab_result_2}.
  Tasks and Datasets are used in existing LMs for scientific text.
  The underlying datasets are those in which the proposed SciLMs outperform previous models or achieve SOTA results.
  }
  \label{tab_result_3}

\resizebox{\textwidth}{!}{%
  \begin{tabular}{p{0.22cm}p{1.9cm}p{5.7cm}p{11cm}}
    \toprule
 \textbf{No.} &   \textbf{Model} & \textbf{Tasks } & \textbf{Datasets}\\







\midrule
\multirow{3}{0.22cm}{36} & \multirow{3}{1.6cm}{BioMedBERT} & \textcolor{blue}{Named Entity Recognition} &  NCBI-disease, BC5CDR-chemical, BC5CDR-disease, BC4CHEMD, BC2GM, JNLPBA \\

  &  & \textcolor{purple}{Relation Extraction} &  GAD, EU-ADR \\
 
&    & \textcolor{orange}{Question Answering} & \underline{BioASQ 5b-factoid}, \underline{BioASQ 6b-factoid}, \underline{BioASQ 7b-factoid}, BioASQ 4b-factoid \\







\midrule
 \multirow{2}{0.3cm}{37} &    \multirow{2}{1.2cm}{LBERT} &  \multirow{2}{4cm}{\textcolor{purple}{Relation Extraction}} & \underline{HPDR50}, \underline{IEPA}, \underline{EU-ADR}, \underline{MedLine}, \underline{BioNLP Shared Task 2011 corpus}, ChemProt, AIMed, BioInfer, GAD, LLL  \\

% &    & \textcolor{purple}{Relation Extraction} & ,  \\ 





\midrule
\multirow{8}{0.3cm}{38} &    \multirow{8}{1.55cm}{OAG-BERT} & \textcolor{Sepia}{Author Name Disambiguation}   &  \underline{whoiswho-v1} \\

 &     & \textcolor{RawSienna}{Scientific Literature Retrieval}  & \underline{OAG-QA} \\

 &     &  \textcolor{Fuchsia}{Paper Recommendation}  & \underline{SciDocs (Recommendation task)} \\

 &     & \textcolor{RubineRed}{User Activity Prediction}   & \underline{Co-Views}, \underline{Co-Reads} \\

 &     &  Entity Graph Completion  & \underline{CS Dataset} \\

 &     &  Fields-of-study Tagging  & \underline{MAG} \\

 &     &  Venue Prediction  &  \underline{arXiv} \\

 &     &  Affiliation Prediction  &  \underline{arXiv} \hl{(All)}  \\







\midrule
\multirow{2}{0.22cm}{39} & \multirow{2}{1.6cm}{CovidBERT} & \textcolor{purple}{Relation Extraction} &  \underline{BioCreative V} \\
% Chemical Disease Relations Recognition

  &  & \textcolor{teal}{Text Classification}  & \underline{DisGeNet Database} \hl{(All)} \\
% 




\midrule
\multirow{3}{0.28cm}{40} & \multirow{3}{1.6cm}{ELECTRAMed} & \textcolor{blue}{Named Entity Recognition} &\underline{BC5CDR},  NCBI-disease, JNLPBA \\

  &  & \textcolor{purple}{Relation Extraction} &  ChemProt, DDI \\
 
&    & \textcolor{orange}{Question Answering} & \underline{BioASQ 7b-factoid} \\






\midrule
\multirow{2}{0.22cm}{41} & \multirow{2}{1.6cm}{KeBioLM} & \textcolor{blue}{Named Entity Recognition} &  \underline{NCBI-disease}, \underline{BC5CDR-chemical}, \underline{BC2GM}, \underline{JNLPBA}, BC5CDR-disease \\

  &  & \textcolor{purple}{Relation Extraction} &  \underline{GAD}, \underline{ChemProt}, DDI \\










\midrule
 \multirow{4}{0.3cm}{42} &    \multirow{4}{1.6cm}{SINA-BERT} & Fill-in-the-Blank  & \underline{10k-sentences}  \\

&    &  \textcolor{teal}{Text Classification}  &  \underline{4k-samples}  \\ 
% Medical Question Classification

&    &  \textcolor{OrangeRed}{Medical Sentiment Analysis}  &  \underline{5k-comments}  \\ 

&    &  \textcolor{RawSienna}{Medical Question Retrieval}  &  \underline{200k-pairs}  \hl{(All)}  \\ 









\midrule
\multirow{3}{0.22cm}{43} & \multirow{3}{2.6cm}{MathBERT (P)} &  \textcolor{RawSienna}{Mathematical Information Retrieval}  &   \underline{NTCIR-12 MathIR} \\

  &  &  Formula Topic Classification  &  \underline{TopicMath-100K}  \\
 
&    &  \textcolor{WildStrawberry}{Formula Headline Generation}   &  \underline{EXEQ-300K} \hl{(All)}  \\









\midrule
 \multirow{2}{0.3cm}{44} &    \multirow{2}{1.2cm}{NukeLM} & OSTI Multi-class Prediction  &  \underline{OSTI subject categories}  \\

&    & OSTI Binary Prediction & \underline{OSTI custom} \hl{(All)}   \\






\midrule
 \multirow{3}{0.3cm}{45} &    \multirow{3}{1.2cm}{ProteinBERT} & Protein Structure   &  Secondary Structure, Disorder, Remote Homology, Fold Classes  \\

&    & Post-translational Modifications  &  Neuropeptide Cleavage, Major PTMs, Signal Peptide  \\

&    &   Biophysical Properties &   \underline{Stability}, Fluorescence \\








\midrule
 \multirow{6}{0.3cm}{46} &    \multirow{6}{1.6cm}{SciFive} &  \multirow{2}{4cm}{\textcolor{blue}{Named Entity Recognition}} &\underline{JNLPBA},  \underline{Species-800}, \underline{BC5CDR-disease}, BC5CDR-chemical, NCBI-disease, BC4CHEMD, BC2GM  \\

  & & \textcolor{purple}{Relation Extraction} & \underline{ChemProt}, \underline{DDI} \\ 

 & & \textcolor{Bittersweet}{Natural Language Inference} &  \underline{MedNLI} \\

& & \textcolor{brown}{Document Multi-label Classification}  & HOC\\

& & \textcolor{orange}{Question Answering}  & \underline{BioASQ 4b-factoid}, \underline{BioASQ 5b-factoid}, \underline{BioASQ 6b-factoid} \\













\midrule
 \multirow{7}{0.3cm}{47} &    \multirow{7}{1.2cm}{BioELECTRA} &  \textcolor{blue}{Named Entity Recognition} & \underline{BC5CDR-chemical}, \underline{BC5CDR-disease}, \underline{JNLPBA}, \underline{NCBI-disease}, \underline{BC2GM}, \underline{ShARe/CLEFE}  \\

  & & \textcolor{purple}{Relation Extraction} & \underline{ChemProt}, \underline{DDI}, \underline{GAD}, \underline{i2b2-2010} \\ 

& & \textcolor{magenta}{PICO Extraction} &  \underline{EBM-NLP}\\

& & \textcolor{Green}{Sentence Similarity} & \underline{BIOSSES}, \underline{ClinicalSTS} \\

& & \textcolor{brown}{Document Multi-label Classification}  & \underline{HOC}\\

& & \textcolor{orange}{Question Answering}  & \underline{PubMedQA}, \underline{BioASQ} \\

 & & \textcolor{Bittersweet}{Natural Language Inference} &  \underline{MedNLI} \hl{(All)} \\








\midrule
 \multirow{2}{0.3cm}{48} &    \multirow{2}{1.6cm}{ChemBERT} & Reaction Role Labeling   &    \underline{Reaction Role Labeling} \\

&    & Product Extraction  &  \underline{Product Extraction}  \hl{(All)} \\






\midrule
 \multirow{4}{0.3cm}{49} &    \multirow{4}{1.6cm}{EntityBERT} &  \textcolor{purple}{Temporal Relation Extraction}  &   \underline{THYME+}  \\

&    &  Document Time Relation Classification & \underline{THYME+}  \\

&    &  Negation Detection & i2b2, MiPACQ, Seed, Strat  \\

&    &  \textcolor{orange}{Question Answering} & PubMedQA  \\






\midrule

\multirow{3}{0.3cm}{50} &    \multirow{3}{2.2cm}{MathBERT (S)} &  Knowledge Component Prediction  &  \underline{ASSISTments} \\

  &   & Auto-grading  &  \underline{ASSISTments} \\

  &   & Knowledge Tracing Correctness Prediction  &  \underline{ASSISTments} \hl{(All)} \\




\midrule
51  &   MedGPT & Next Disorder Prediction  &  \underline{MIMIC-III}, \underline{KTH}  \hl{(All)} \\ 






  \bottomrule
\end{tabular}
}

\end{table}


==> tables/scilms_results_04.tex <==





% Table result - 4
\begin{table}

  \caption{
  A continuation of the table from Tables \ref{tab_result_1}, \ref{tab_result_2}, and \ref{tab_result_3}.
  Tasks and Datasets are used in existing LMs for scientific text.
  The underlying datasets are those in which the proposed SciLMs outperform previous models or achieve SOTA results.
  }
  \label{tab_result_4}

\resizebox{\textwidth}{!}{%
  \begin{tabular}{p{0.22cm}p{2.3cm}p{5.4cm}p{10.4cm}}
    \toprule
 \textbf{No.} &   \textbf{Model} & \textbf{Tasks } & \textbf{Datasets}\\









\midrule
 \multirow{6}{0.3cm}{52} &    \multirow{6}{1.6cm}{SMedBERT} &  \textcolor{blue}{Named Entity Recognition} &  \underline{cMedQANER}, \underline{DXY-NER} \\

  & & \textcolor{purple}{Relation Extraction} & \underline{DXY-RE}, \underline{CHIP-RE} \\ 

& & \textcolor{magenta}{Question Matching} &  \underline{cMedQQ}\\

& & \textcolor{Mahogany}{Intrinsic Evaluation}  & \underline{D1}, \underline{D2}, \underline{D3} \\

& & \textcolor{orange}{Question Answering}  & \underline{cMedQA}, \underline{WebMedQA} \\

 & & \textcolor{Bittersweet}{Natural Language Inference} &  \underline{cMedNLI} \hl{(All)} \\





\midrule
 53 &  Bio-cli   &  \textcolor{blue}{Named Entity Recognition}  &  \underline{PharmaCoNER}, CANTEMIST, \underline{ICTUSnet} \\
 





\midrule
 \multirow{3}{0.3cm}{54} &    \multirow{3}{1.6cm}{MatSciBERT} & \textcolor{blue}{Named Entity Recognition}  &  \underline{SOFC}, \underline{SOFC-Slot}, \underline{Matscholar NER} \\

  & & \textcolor{teal}{Text Classification}  &  \underline{Glass vs. Non-glass Dataset} \\ 

  & & \textcolor{purple}{Relation Extraction}  &  \underline{Materials Synthesis Procedures Dataset} \hl{(All)} \\ 









\midrule
\multirow{2}{0.3cm}{55}  &   \multirow{2}{1.6cm}{ClimateBert} &  \textcolor{teal}{Text Classification}  &  \underline{Climate-related Classification} \\ 

&    &  \textcolor{OrangeRed}{Sentiment Analysis}  &  \underline{Climate-related Paragraphs} \hl{(All)} \\ 




 

\midrule
\multirow{2}{0.3cm}{56}  &   \multirow{2}{1.6cm}{MatBERT} &  \multirow{2}{4.6cm}{\textcolor{blue}{Named Entity Recognition}}  &  \underline{Solid-state Materials Abstracts}, \underline{Inorganic Doping Abstracts}, \underline{Gold Nanoparticle Synthesis}  \hl{(All)} \\ 





\midrule
57  &   UTH-BERT   &  MedWeb Task (8 labels)  &  \underline{MedWeb} \hl{(All)} \\ 






\midrule
58  &  ChestXRayBERT  &  \textcolor{Plum}{Summarization}  &  \underline{OPEN-I}, \underline{MIMIC-CXR} \hl{(All)} \\ 







\midrule
 \multirow{3}{0.3cm}{59} &    \multirow{3}{1.2cm}{MedRoBERTa.nl} &  Medical Odd-one-out Similarity Task & \underline{Medical odd-one-out Similarity Task}  \\

  & & ICF Classification Task & ICF Classification Task \\ 

  & & \textcolor{blue}{Named Entity Recognition} (Dutch) & CoNLL 2002 \\ 





\midrule
 \multirow{6}{0.3cm}{60} &    \multirow{6}{1.2cm}{PubMedELECTRA} &  \textcolor{blue}{Named Entity Recognition} &  BC5CDR-chemical, JNLPBA, NCBI-disease, BC5CDR-disease, BC2GM \\

  & & \textcolor{purple}{Relation Extraction} &  \underline{GAD}, ChemProt, DDI  \\ 

& & \textcolor{magenta}{PICO Extraction} &  \underline{EBM-NLP} \\

& & \textcolor{Green}{Sentence Similarity} &  BIOSSES \\

& & \textcolor{brown}{Document Multi-label Classification}  & HOC  \\

& & \textcolor{orange}{Question Answering}  &  PubMedQA, BioASQ \\







\midrule
 \multirow{4}{0.3cm}{61} &      \multirow{4}{1.2cm}{Clinical-Longformer} &  \textcolor{blue}{Named Entity Recognition} & \underline{i2b2 2006}, \underline{i2b2 2010}, \underline{i2b2 2012}, \underline{i2b2 2014}  \\

& & \textcolor{teal}{Text Classification}  & \underline{MIMIC-AKI}, \underline{OpenI}, OHSUMed\\

& & \textcolor{orange}{Question Answering}  & \underline{emrQA} \\

 & & \textcolor{Bittersweet}{Natural Language Inference} &  \underline{MedNLI} \\

% \multirow{4}{1.2cm}{Clinical-BigBird} &  \textcolor{blue}{Named Entity Recognition} & i2b2 2006, i2b2 2010, i2b2 2012, i2b2 2014  \\

% & & \textcolor{OliveGreen}{Document Classification}  & MIMIC-AKI, OpenI, OHSUMed\\

% & & \textcolor{orange}{Question Answering}  & emrQA \\

%  & & \textcolor{Bittersweet}{Natural Language Inference} &  MedNLI \\




\midrule
 \multirow{6}{0.3cm}{62} &    \multirow{6}{1.2cm}{BioLinkBERT} &  \textcolor{blue}{Named Entity Recognition} &  \underline{BC5CDR-chemical},  \underline{BC5CDR-disease}, \underline{JNLPBA}, \underline{NCBI-disease}, \underline{BC2GM} \\

  & & \textcolor{purple}{Relation Extraction} &  \underline{GAD}, \underline{ChemProt}, \underline{DDI}  \\ 

& & \textcolor{magenta}{PICO Extraction} &  \underline{EBM-NLP} \\

& & \textcolor{Green}{Sentence Similarity} &  \underline{BIOSSES} \\

& & \textcolor{brown}{Document Multi-label Classification}  & \underline{HOC}  \\

& & \textcolor{orange}{Question Answering}  &  \underline{PubMedQA}, \underline{BioASQ} \hl{(All)} \\




\midrule
 \multirow{4}{0.3cm}{63} &    \multirow{4}{1.2cm}{BioBART} &  \textcolor{blue}{Named Entity Recognition} & ShARe13, ShARe14, CADEC, GENIA \\

  & & \textcolor{Apricot}{Entity Linking} &  \underline{BC5CDR}, \underline{AskAPatient}, \underline{COMETA}, MedMentions, NCBI-disease  \\ 

& & \textcolor{Plum}{Summarization} &  \underline{MeQSum}, \underline{MEDIQA-ANS}, iCliniq, HealthCareMagic,  MEDIQA-QS, MEDIQA-MAS \\

& & \textcolor{RoyalBlue}{Dialogue} & \underline{CovidDialog} \\





\midrule
\multirow{2}{0.3cm}{64} &    \multirow{2}{1.2cm}{SecureBERT} &  \textcolor{blue}{Named Entity Recognition} & \underline{MalwareTextDB}  \\

  % &    &  MLM &   \underline{17k-records} \\ 

  &    &  \textcolor{OrangeRed}{Sentiment Analysis} &  Rotten Tomatoes  \\ 


\midrule
 \multirow{2}{0.3cm}{65} &    \multirow{2}{1.2cm}{BatteryBERT} &  \textcolor{orange}{Question Answering} & Retional Data Extraction, Device Component Classification \\

& & \textcolor{teal}{Text Classification} & Battery Abstract Classification \\





\midrule
66  &   bsc-bio-ehr-es  &  \textcolor{blue}{Named Entity Recognition} &  \underline{PharmaCoNER}, \underline{CANTEMIST}, \underline{ICTUSnet} \hl{(All)} \\ 




\midrule
67  &   ChemGPT  &  N/A  &  N/A  \\ 






% \midrule
%  \multirow{2}{0.3cm}{68} &    \multirow{2}{1.2cm}{PathologyBERT} &   Masked Language Prediction & \underline{Unlabeled pathology reports}, \underline{Manually labeled pathology reports}  \\


% & & Cancer Severity Classification  & \underline{Breast Cancer Diagnose Severity Classification}  \hl{(All)} \\



\midrule
 \multirow{1}{0.3cm}{68} &    \multirow{1}{1.2cm}{PathologyBERT} &  Cancer Severity Classification  & \underline{Breast Cancer Diagnose Severity Classification}  \hl{(All)} \\




\midrule
 \multirow{3}{0.3cm}{69} &    \multirow{3}{1.2cm}{ScholarBERT} &   \multirow{2}{4.6cm}{\textcolor{blue}{Named Entity Recognition}} & \underline{ScienceExam}, SciERC, NCBI-disease, 
ChemDNER, Matscholar NER, BC5CDR, JNLPBA,  Coleridge \\

  & & \textcolor{purple}{Relation Extraction} & \underline{SciERC}, ChemProt, Paper Field \\ 





\midrule
 \multirow{3}{0.3cm}{70} &    \multirow{3}{1.2cm}{RadBERT} &   \textcolor{teal}{Text Classification} & \underline{Abnormal Sentence Classification} \\

  & & Report Coding & \underline{AAA}, \underline{BI-RADS}, \underline{Lung-RADS}, \underline{Abnormal}, \underline{Alert} \\ 

  & & \textcolor{Plum}{Summarization} &  \underline{Summarization} \hl{(All)} \\ 






  \bottomrule
\end{tabular}
}

\end{table}



==> tables/scilms_results_05.tex <==

% Table result - 5
\begin{table}

  \caption{
  A continuation of the table from Tables \ref{tab_result_1}, \ref{tab_result_2}, \ref{tab_result_3}, and \ref{tab_result_4}.
  Tasks and Datasets are used in existing LMs for scientific text.
  The underlying datasets are those in which the proposed SciLMs outperform previous models or achieve SOTA results.
  }
  \label{tab_result_5}

\resizebox{\textwidth}{!}{%
  \begin{tabular}{p{0.22cm}p{2.4cm}p{6.2cm}p{10.2cm}}
    \toprule
 \textbf{No.} &   \textbf{Model} & \textbf{Tasks } & \textbf{Datasets}\\










\midrule
 \multirow{3}{0.3cm}{71} &    \multirow{3}{1.2cm}{SciDeBERTa} &   \textcolor{blue}{Named Entity Recognition} & \underline{SciERC}, \underline{GENIA} \\

  & & \textcolor{purple}{Relation Extraction} & \underline{SciERC} \\ 

  & & Co-reference Resolution & \underline{GENIA}, SciERC  \\ 




\midrule
 \multirow{4}{0.3cm}{72} &    \multirow{4}{1.2cm}{SsciBERT} &  \textcolor{blue}{Named Entity Recognition}  & \underline{Scientometrics} \\

  & & Identification Results of Abstract Structures & \underline{Identification Results of Abstract Structures} \\ 

  & & Discipline Classification & \underline{JCR Social Science} \hl{(All)} \\ 







\midrule  
\multirow{3}{0.3cm}{73} &    \multirow{3}{1.2cm}{ViHealthBERT} &  \textcolor{blue}{Named Entity Recognition}   &  \underline{COVID-19}, \underline{ViMQ} \\

  & & \textcolor{Sepia}{Acronym Disambiguation Task} &  \underline{acrDrAid}  \\ 

  & & \textcolor{Plum}{Summarization} &  \underline{FAQ Summarization} \hl{(All)} \\ 







\midrule
74  &   Clinical Flair  & \textcolor{blue}{Named Entity Recognition}  &   \underline{CANTEMIST}, \underline{Clinical Trials}, \underline{NUBes}, PharmaCoNER  \\ 





\midrule
 \multirow{2}{0.3cm}{75} &    \multirow{2}{1.6cm}{KM-BERT} &  \textcolor{blue}{Named Entity Recognition}  & \underline{Korean NER} \\

  & & \textcolor{MidnightBlue}{Semantic Textual Similarity}  & \underline{Korean MedSTS} \hl{(All)} \\ 




 
\midrule
76  &   MaterialsBERT (S) & \textcolor{blue}{Named Entity Recognition}  & \underline{A polymer dataset annotated by the authors} \hl{(All)} \\ 




\midrule
77  &   ProcessBERT & \textcolor{teal}{Text Classification}    &    \underline{Phrases manually annotated dataset} \hl{(All)} \\ 






\midrule
 \multirow{4}{0.3cm}{78} &    \multirow{4}{1.2cm}{BioGPT} &  \textcolor{WildStrawberry}{Generation} & Self-created Text Generation Dataset \\

  & & \textcolor{purple}{Relation Extraction} & \underline{BC5CDR}, \underline{KD-DTI}, \underline{DDI} \\ 

& & \textcolor{brown}{Document Multi-label Classification}  & \underline{HOC} \\

& & \textcolor{orange}{Question Answering}  & \underline{PubMedQA}\\






\midrule
 \multirow{2}{0.3cm}{79} &    \multirow{2}{2.3cm}{ChemBERTa-2} &  Classification  & \underline{BBBP}, \underline{SR-p53}, BACE,  ClinTox \\

  & & Regression & \underline{Clearance}, \underline{Delaney}, \underline{Lipo}, BACE \\ 







\midrule
 \multirow{3}{0.3cm}{80} &    \multirow{3}{1.2cm}{CSL-T5} &  \textcolor{Plum}{Summarization} &  \underline{Predict Title from Abstract} (Created by authors) \\

  & & \textcolor{WildStrawberry}{Generation} & \underline{Chinese Keyword Generation Task} (Created by authors) \\ 

& & \textcolor{teal}{Text Classification}  & \underline{CTG}, \underline{DCP} (Created by authors) \hl{(All)}  \\







\midrule
 \multirow{2}{0.3cm}{81} &    \multirow{2}{2.8cm}{MaterialBERT (Y)} &  Visualization of Materials  & Visualization of Materials \\

  & & \textcolor{teal}{Text Classification} & CoLA \\ 





 \midrule
\multirow{1}{0.3cm}{82} &    \multirow{1}{1.8cm}{AcademicRoBERTa} &  \textcolor{teal}{Text Classification}  &  \underline{Author Identification}, \underline{Category Classification} \hl{(All)} \\

 % &     &  Category Classification   &  \\




 \midrule
 83 &  Bioberturk   &  \textcolor{teal}{Radiology Report classification}  &  \underline{Impressions}, \underline{Findings} \hl{(All)}\\








\midrule
84  &   DRAGON & \textcolor{orange}{Question Answering}   &    \underline{MedQA}, \underline{PubMedQA}, \underline{BioASQ} \hl{(All)} \\ 





\midrule
 \multirow{5}{0.3cm}{85} &    \multirow{5}{1.8cm}{UCSF-BERT} &  \textcolor{blue}{Named Entity Recognition} & \underline{i2b2 2010}, i2b2 2012   \\

  & & \textcolor{purple}{Relation Extraction} & \underline{i2b2 2010} \\ 

& & \textcolor{Bittersweet}{Natural Language Inference} & MedNLI \\

& & ICD9-top50 Coding & \underline{ICD9-top50 Coding} \\

& & Therapeutic Class Prediction  & \underline{Therapeutic Class Prediction} \\




\midrule  
\multirow{3}{0.3cm}{86} &    \multirow{3}{1.2cm}{ViPubmedT5} &  \textcolor{Bittersweet}{Natural Language Inference}   &   \underline{ViMedNLI} \\

  & & \textcolor{Sepia}{Acronym Disambiguation Task} &  \underline{acrDrAid}  \\ 

  & & \textcolor{Plum}{Summarization}  &  FAQ Summarization \\ 













\midrule
 \multirow{9}{0.3cm}{87} &    \multirow{9}{1.8cm}{Galactica} & General Capabilities  & \underline{57 task selection from BIG-bench} \\

 % \cmidrule{3-4}
  &    &  Downstream Scientific NLP  &  \underline{MMLU benchmark}, \underline{other popular scientific QA benchmarks}  \\ 



 % \cmidrule{3-4}
  &    &  Citation Prediction  &  \underline{Citation Accuracy} (PWC Citations, Extended Citations, Contextual Citations)  \\ 
 % \cmidrule{3-4}

  &    &  Chemical Understanding  &  \underline{IUPAC Name Prediction}, MoleculeNet  \\ 
  
  &    &  Toxicity and Bias  &  \underline{Bias and Stereotypes} (CrowS-Pairs, StereoSet, Toxicity), \underline{TruthfulQA}  \\


 \cmidrule{3-4}
  &    &  \multirow{2}{4.6cm}{Knowledge Probes}  &  \underline{LaTeX Equations}, Domain Probes (\underline{AminoProbe}, BioLAMA, \underline{Chemical Reactions}, \underline{Galaxy Clusters}, \underline{Mineral Groups}), Reasoning (\underline{MMLU Mathematics}, MATH)  \\ 


 \cmidrule{3-4}
  &    &  \multirow{2}{4.6cm}{Biological Understanding}  &  \underline{Sequence Validation Perplexity}, \underline{Protein Keyword Prediction}, \underline{Protein Function Description}  \\ 
 % \cmidrule{3-4}
 



\midrule
 \multirow{4}{0.3cm}{88} &    \multirow{4}{1.8cm}{VarMAE} &  \textcolor{blue}{Named Entity Recognition} & \underline{JNLPBA}, \underline{IEE} \\

  & & \textcolor{teal}{Text Classification} & \underline{ACL-ARC}, \underline{SciCite}, \underline{OIR}, \underline{MTC}\\ 

& & \textcolor{magenta}{PICO Extraction} &  \underline{EBM-NLP} \\

& & Text Matching & \underline{PSM} \hl{(All)} \\






\midrule
89  &   AliBERT  & \textcolor{blue}{Named Entity Recognition}  &  \underline{BioNER}, \underline{QUAERO}  \hl{(All)} \\     





\midrule
 \multirow{2}{0.3cm}{90} &    \multirow{2}{1.8cm}{BioMedLM} &  \textcolor{WildStrawberry}{Text Generation} & MeQSum \\
& & \textcolor{orange}{Question Answering}  & \underline{MedQA}, PubMedQA, and BioASQ \\












  \bottomrule
\end{tabular}
}

\end{table}




==> tables/scilms_results_06.tex <==

% Table result - 6
\begin{table}

  \caption{
  A continuation of the table from Tables \ref{tab_result_1}, \ref{tab_result_2}, \ref{tab_result_3}, \ref{tab_result_4}, and \ref{tab_result_5}.
  Tasks and Datasets are used in existing LMs for scientific text.
  The underlying datasets are those in which the proposed SciLMs outperform previous models or achieve SOTA results.
  }
  \label{tab_result_6}

\resizebox{\textwidth}{!}{%
  \begin{tabular}{p{0.22cm}p{2.0cm}p{5.4cm}p{9.6cm}}
    \toprule
 \textbf{No.} &   \textbf{Model} & \textbf{Tasks } & \textbf{Datasets}\\








\midrule
 \multirow{6}{0.3cm}{91} &    \multirow{6}{1.8cm}{BioReader} &  \multirow{2}{4.4cm}{\textcolor{blue}{Named Entity Recognition}} & \underline{BC4CHEMD}, \underline{Species-800}, JNLPBA, NCBI-disease, BC5CDR-disease, BC5CDR-chemical, 
BC2GM  \\

  & & \textcolor{purple}{Relation Extraction} & ChemProt, \underline{DDI} \\ 

& & \textcolor{brown}{Document Multi-label Classification}  & \underline{HOC} \\

& & \textcolor{orange}{Question Answering}  & BioASQ 4b-factoid, BioASQ 5b-factoid, BioASQ 6b-factoid, MedQA-USMLE  \\

& & \textcolor{Bittersweet}{Natural Language Inference} & MedNLI \\







\midrule
 \multirow{4}{0.3cm}{92} &    \multirow{4}{1.8cm}{ClinicalT5} &  \textcolor{blue}{Named Entity Recognition} & \underline{NCBI-disease}, BC5CDR-disease  \\

  & & \textcolor{Mahogany}{Intrinsic Evaluation} & UMNSRS-Sim, UMNSRS-Rel \\ 

& & \textcolor{brown}{Document Multi-label Classification}  & \underline{HOC} \\

& & \textcolor{Bittersweet}{Natural Language Inference} & \underline{MedNLI} \\






\midrule   

 \multirow{5}{0.3cm}{93} &    \multirow{5}{1.8cm}{CySecBERT} &  \textcolor{blue}{Named Entity Recognition} &  \underline{NVD}  \\ 

  &      &  Word Similarity Task  &  \underline{Word Similarity}  \\ 

  &      &   Clustering Task  &  \underline{Log4J dataset}  \\ 


  &      &  Classification &  \underline{CySecAlert},  \underline{MS Exchange}  \\ 

  &      &  Combined Task &  SuperGLUE  \\ 






\midrule
 \multirow{5}{0.3cm}{94} &    \multirow{5}{1.2cm}{GatorTron} &  \textcolor{blue}{Named Entity Recognition} &  \underline{i2b2 2010},  \underline{i2b2 2012}, \underline{n2c2 2018} \\

  & & \textcolor{purple}{Relation Extraction} & \underline{n2c2 2018} \\ 

  & & \textcolor{MidnightBlue}{Semantic Textual Similarity}  & \underline{n2c2 2019} \\ 

& & \textcolor{Bittersweet}{Natural Language Inference} & \underline{MedNLI} \\

  & & \textcolor{orange}{Medical Question Answering} & \underline{emrQA}  \hl{(All)} \\  








\midrule
 \multirow{2}{0.3cm}{95} &    \multirow{2}{1.8cm}{Med-PaLM} &  \multirow{2}{4.4cm}{\textcolor{orange}{Question Answering}} & \underline{MedQA-USMLE}, \underline{MedMCQA}, \underline{PubMedQA}, MMLU, LiveQA, MedicationQA, HealthSearchQA  \\







\midrule
96  &   Clinical-T5  & N/A  &  N/A  \\ 





\midrule
\multirow{1}{0.3cm}{97}  &    \multirow{1}{4.2cm}{CPT-BigBird}  & \multirow{1}{4.4cm}{\textcolor{orange}{Question Answering}}  &  \multirow{1}{5.3cm}{SQuAD, IS-QA}  \\ 








\midrule
 \multirow{3}{0.3cm}{98} &    \multirow{3}{1.8cm}{ProtST} &  Protein Localization Prediction &  \underline{Bin}, \underline{Sub} \\

& &  Fitness Landscape Prediction  &  \underline{$\beta$-lac}, \underline{AAV}, \underline{Thermo}, \underline{Flu}, \underline{Sta}    \\ 
  
& &   Protein Function Annotation    &   \underline{EC}, \underline{GO-BP}, \underline{GO-MF}, \underline{GO-CC}  \hl{(All)}    \\






\midrule
\multirow{2}{0.3cm}{99}  &   \multirow{2}{2.5cm}{SciEdBERT}   & Automatic Scoring of Students' Written Responses   &  \multirow{2}{5cm}{\underline{4T}, \underline{7T}  \hl{(All)}} \\ 



% \midrule
%  \multirow{3}{0.3cm}{98} &    \multirow{3}{1.8cm}{ProtST} &   &   \\

% & &   &      \\ 
  
% & &       &       \\




\midrule
 \multirow{4}{0.3cm}{100} &    \multirow{4}{1.8cm}{Bioformer} &  \multirow{2}{4.4cm}{\textcolor{blue}{Named Entity Recognition}} & BC5CDR-disease, NCBI-disease, BC5CDR-chemical, BC4CHEMD, BC2GM, JNLPBA, LINNAEUS, Species-800  \\

& & \textcolor{purple}{Relation Extraction} & ChemProt, DDI, EU-ADR, GAD \\ 
  
& & \textcolor{brown}{Document Multi-label Classification}  & HOC, BioCreative-LitCovid \\









\midrule
 \multirow{4}{0.3cm}{101} &    \multirow{4}{1.8cm}{Lightweight Clinical Transformers} &  \textcolor{blue}{Named Entity Recognition} &  \underline{i2b2 2010}, i2b2 2012, \underline{i2b2 2014}   \\

& & \textcolor{purple}{Relation Extraction} & \underline{i2b2 2010} \\ 
  
& & \textcolor{Bittersweet}{Natural Language Inference}  & MedNLI \\


& & Sequence Classification  &  \underline{Isaric Clinical Notes (ICN)} \\







\midrule
102  &   ManuBERT   &  \textcolor{blue}{Named Entity Recognition} &  \underline{FabNER}  \\ 





\midrule
103  &   RAMM   &   \textcolor{orange}{Visual Question Answering}  &  \underline{Med-VQA 2019}, \underline{VQA-Med 2021}, \underline{VQARAD}, \underline{SLAKE}  \hl{(All)} \\ 







\midrule
 \multirow{5}{0.3cm}{104} &    \multirow{5}{1.8cm}{DrBERT} & \multirow{2}{4cm}{\textcolor{blue}{Named Entity Recognition}}   & \underline{MUSCA-DET}, \underline{QUAERO-EMEA}, \underline{QUAERO-MEDLINE}, \underline{Acute heart failure (aHF)}, \underline{Medical Report}   \\  


&     &   \textcolor{teal}{Text Classification}   & \underline{aHF}, \underline{MUSCA-DET}, \underline{Technical Specialties Sorting}   \\ 

&     &   POS Tagging & \underline{ESSAIS}, CAS  \\


&     &  \textcolor{orange}{Question Answering}    &  FrenchMedMCQA \\ 









\midrule
 \multirow{4}{0.3cm}{105} &    \multirow{4}{1.8cm}{MOTOR} & \textcolor{WildStrawberry}{Medical Report Generation}  &  \underline{IU-Xray} \\

& & \textcolor{RawSienna}{Image Report Retrieval}  &  \underline{MIMIC-CXR}    \\ 
  
& &   Diagnosis Classification    &   \underline{MIMIC-CXR}, ChestX-ray14    \\

& &   \textcolor{orange}{Visual Question Answering}    &    \underline{SLAKE}, VQARAD   \\














  \bottomrule
\end{tabular}
}

\end{table}



==> tables/scilms_results_07.tex <==

% Table result - 7
\begin{table}

  \caption{
  A continuation of the table from Tables \ref{tab_result_1}, \ref{tab_result_2}, \ref{tab_result_3}, \ref{tab_result_4},  \ref{tab_result_5}, and \ref{tab_result_6}.
  Tasks and Datasets are used in existing LMs for scientific text.
  The underlying datasets are those in which the proposed SciLMs outperform previous models or achieve SOTA results.
  }
  \label{tab_result_7}

\resizebox{\textwidth}{!}{%
  \begin{tabular}{p{0.22cm}p{2.4cm}p{5.4cm}p{9.9cm}}
    \toprule
 \textbf{No.} &   \textbf{Model} & \textbf{Tasks } & \textbf{Datasets}\\






\midrule
 \multirow{5}{0.3cm}{106} &    \multirow{5}{1.8cm}{BiomedGPT} &  Image Classification & \underline{MedMNIST v2}  \\

& & \textcolor{Bittersweet}{Natural Language Inference} &  MedNLI \\ 

& & \textcolor{Plum}{Summarization} &  MeQSum, iCliniq, HealthCareMagic \\ 

& & \textcolor{Emerald}{Image Captioning} & \underline{Peir Gross}, IU X-ray, ROCO \\ 

& & \textcolor{orange}{Visual Question Answering} &  \underline{SLAKE}, \underline{PathVQA}, VQARAD \\ 








\midrule
 \multirow{4}{0.3cm}{107} &    \multirow{4}{1.8cm}{Patton} &  Classification  &  PATTON (\underline{Mathematics, Clothes, Sports}), SciPATTON (\underline{Geology, Economics}) \\

& & Retrieval  &  PATTON (\underline{Clothes, Sports}), SciPATTON (\underline{Mathematics, Geology, Economics})    \\ 
  
& &  Reranking     &    PATTON (\underline{Clothes, Sports}), SciPATTON (\underline{Mathematics, Geology, Economics})   \\

& &    Link Prediction   &    SciPATTON (\underline{Mathematics, Geology, Economics})   \\







\midrule
108  &   TurkRadBERT   & \textcolor{teal}{Text Classification}  &  Turkish head CT reports  \\ 





\midrule
109  &   CamemBERT-bio   & \textcolor{blue}{Named Entity Recognition}  &  \underline{CAS1}, \underline{CAS2}, \underline{QUAERO-EMEA}, QUAERO-MEDLINE, E3C  \\ 







\midrule
 \multirow{4}{0.3cm}{110} &    \multirow{4}{1.8cm}{ClinicalGPT} &  \textcolor{RoyalBlue}{Medical Conversation} & \underline{MedDialog}  \\


& & Diagnosis & \underline{MD-EHR}  \\ 

& &  \textcolor{orange}{Medical Question Answering} & \underline{cMedQA2}, MEDQA-MCMLE  \\ 






\midrule

\multirow{3}{0.3cm}{111} &    \multirow{3}{1.8cm}{EriBERTa} & \multirow{2}{4.6cm}{\textcolor{blue}{Named Entity Recognition}}  &  BC5CDR-disease, BC5CDR-chemical, JNLPBA, NCBI-disease, BC4CHEM, DIANN, Treatment \\ 

& & \textcolor{blue}{Named Entity Recognition} (Spanish)  &   \underline{PharmaCoNER}, \underline{Cantemist-NER}   \\ 





\midrule
 \multirow{1}{0.3cm}{112} &    \multirow{1}{1.8cm}{K2} & \textcolor{orange}{Question Answering}  &  \underline{NPEE}, APTest \\





% \midrule
%  \multirow{2}{0.3cm}{112} &    \multirow{2}{1.8cm}{K2} & Objective Tasks in GeoBench  &  \underline{NPEE}, APTest \\

% & & Subjective Tasks in GeoBench   &  \underline{Perplexity}, GPTScore, \underline{Rationality}, \underline{Correctness}, Consistency (5 measurements)   \\ 





\midrule
 \multirow{3}{0.3cm}{113} &    \multirow{3}{1.8cm}{PharmBERT} & \multirow{2}{4.8cm}{Drug Labeling}  &  \underline{Detection of adverse drug reaction}, \underline{Extraction of drug–drug interaction}, \underline{ADME classification} \\

& &  \textcolor{OrangeRed}{Sentiment Labeling}  &  SST-2    \\ 





\midrule

 \multirow{2}{0.3cm}{114} &    \multirow{2}{1.8cm}{BioNART} & \textcolor{Plum}{Summarization}  &  iCliniq, HealthCareMagic \\ 

& &  \textcolor{RoyalBlue}{Clinical Dialogue}  &  CovidDialog    \\ 





\midrule
115  &   BIOptimus   & \textcolor{blue}{Named Entity Recognition}  &  \underline{BC5-chemical}, \underline{NCBI-disease}, \underline{BC2GM}, BC5-disease, JNLPBA  \\ 








\midrule
 \multirow{3}{0.3cm}{116} &    \multirow{3}{1.8cm}{KEBLM} & \textcolor{Apricot}{Entity Linking}  & \underline{COMETA}, \underline{NCBI-disease}, BC5CDR-chemical, BC5CDR-disease  \\

& &  \textcolor{Bittersweet}{Natural Language Inference} &   \underline{MedNLI}   \\ 
  
& &    \textcolor{orange}{Question Answering}   &   \underline{PubMedQA}    \\







\midrule
 \multirow{4}{0.3cm}{117} &    \multirow{4}{1.8cm}{GIT-Mol} & \textcolor{Emerald}{Captioning}  & \underline{Molecule Captioning}, \underline{Molecule Image Captioning}   \\

& & \textcolor{WildStrawberry}{Molecule Generation}  &  \underline{Molecule Generation}    \\ 
  

& &  Molecular Property Prediction     &    \underline{ToxCast}, \underline{Sider}, \underline{ClinTox}, \underline{Bace},  \underline{BBBP}, Tox21   \\








  \bottomrule
\end{tabular}
}

\end{table}


==> tables/type_of_architecture.tex <==
\begin{table}

  \caption{
Four types of architectures and a list of SciLMs. 
  }
  \label{type_of_architecture}
 % \resizebox{\textwidth}{!}{%
  \begin{tabular}{l c p{2.4cm} p{11cm}}
    \toprule
  \textbf{Type of Architecture} &  \textbf{List of SciLMs}  \\
    \midrule


\multirow{20}{2.4cm}{Encoder-only}  &  \multirow{20}{11cm}{
BioBERT, BERT-MIMIC, SciBERT, Clinical BERT (Emily), ClinicalBERT (Kexin), BlueBERT, BEHRT, EhrBERT, S2ORC-SciBERT, Clinical XLNet, NukeBERT, GreenBioBERT, SPECTER, BERT-XML, Bio-ELECTRA, Med-BERT, ouBioBERT, PubMedBERT, MC-BERT, BioALBERT, BRLTM, BioMegatron, CharacterBERT, ChemBERTa, ClinicalTransformer, SapBERT, UmlsBERT, bert-for-radiology, Bio-LM, CODER, exBERT, BioMedBERT, LBERT, OAG-BERT, CovidBERT, ELECTRAMed, KeBioLM, SINA-BERT, MathBERT (Peng), NukeLM, BioELECTRA, ChemBERT, EntityBERT, MathBERT (Shen), Bio-cli, MatSciBERT, ClimateBert, MatBERT, UTH-BERT, ChestXRayBERT, MedRoBERTa.nl, PubMedELECTRA, Clinical-Longformer, BioLinkBERT, SecureBERT, BatteryBERT, bsc-bio-ehr-es, PathologyBERT, ScholarBERT, RadBERT, SsciBERT, ViHealthBERT, KM-BERT, MaterialsBERT (Shetty), ProcessBERT, ChemBERTa-2, MaterialBERT (Yoshitake), AcademicRoBERTa, Bioberturk, UCSF-BERT, VarMAE, ALIBERT, CySecBERT, Gatortron, CPT-BigBird, ProtST, SciEdBERT, Bioformer, Lightweight Clinical Transformers, ManuBERT, RAMM, DrBERT, TurkRadBERT, CamemBERT-bio, EriBERTa, PharmBERT, BIOptimus, KEBLM
} \\ \\ \\ \\ \\ \\ \\ \\ \\ \\ \\ \\ \\ \\ \\ \\ \\ \\  \\ \\ 




\midrule
\multirow{5}{2.4cm}{Decoder-only}  &  \multirow{5}{11cm}{Knowledge Graph Construction Knowledge \\ Graph Construction Knowledge Graph Construction \\ Knowledge Graph Construction} \\ \\ \\ \\ \\ \\ 


\midrule
\multirow{5}{2.4cm}{Encoder-Decoder}  &  \multirow{5}{11cm}{Knowledge Graph Construction Knowledge \\ Graph Construction Knowledge Graph Construction \\ Knowledge Graph Construction} \\ \\ \\ \\ \\ \\ 



\midrule
\multirow{5}{2.4cm}{Other types of LMs}  &  \multirow{5}{11cm}{Knowledge Graph Construction Knowledge \\ Graph Construction Knowledge Graph Construction \\ Knowledge Graph Construction} \\ \\ \\ \\ \\ \\ 


 
  \bottomrule
\end{tabular}
% }
\end{table}

